The Dependence of the Type Ia Supernova Host Bias on Observation or Fitting Technique

More luminous Type Ia supernovae (SNe Ia) prefer less massive hosts and regions of higher star formation. This correlation is inverted during width-color-luminosity light curve standardization resulting in step-like biases of distance measurements with respect to host properties. Using the PISCO supernova host sample and SDSS, GALEX, and 2MASS photometry, we compare host stellar mass and specific star formation rate (sSFR) from different observation methods, including local vs. global, and fitting techniques to measure their impact on the host step biases. Mass step measurements for all our mass samples are consistent within a 1$\sigma$ significance from -0.03$\pm$0.02 mag to -0.04$\pm$0.02 mag. Including or excluding UV information had no effect on measured mass step size or location. Specific SFR (sSFR) step sizes are more significant than mass step measurements and varied from $0.05\pm0.03$ mag (H$\alpha$) and $0.06\pm0.02$ mag (UV) for a 51 host sample. The sSFR step location is influenced by mass sample used to normalize star formation and by sSFR tracer choice. The step size is reduced to 0.04$\pm$0.03 mag when using all available 73 hosts with H$\alpha$ measurements. This 73 PISCO host subsample overall lacked a clear step signal, but here we are searching for whether different choices of mass or sSFR estimation can create a step signal. We find no evidence that different observation or fitting techniques choice can create a distance measurement step in either mass or sSFR.

==> gal_master_full.tex <==
\begin{deluxetable}{lrrrccccc}
\tablecaption{Galaxy coverage and fit successes. All photometry mass fits were successful.} \rotate \label{table:coverage}
\tablehead{\colhead{Galaxy} & \colhead{RA} & \colhead{Dec} & \colhead{$z$} & \colhead{GALEX} & \colhead{SDSS} & \colhead{2MASS} & \colhead{SFR} & \colhead{STARLIGHT Mass}}
\startdata
2MASSJ00164451 & 4.185 & 15.342 & 0.070 & X & X & X &  & X \\
2MASSJ00235669 & 5.986 & 29.522 & 0.073 & X & X & X &  & X \\
2MASSJ23243021 & 351.126 & 14.651 & 0.042 & X & X & X &  & X \\
2MASXJ22532475 & 343.353 & 4.799 & 0.024 & X & X & X & X & X \\
2MASXJ00234829 & 5.951 & -3.856 & 0.054 & X & X & X & X & X \\
2MASXJ01144386 & 18.683 & 0.286 & 0.045 & X & X & X & X & X \\
2MASXJ01403375 & 25.141 & 18.511 & 0.064 & X & X & X &  & X \\
2MASXJ02305208 & 37.717 & 22.476 & 0.031 & X & X & X &  & X \\
2MASXJ04424248 & 70.677 & 18.583 & 0.016 & X & X & X &  & X \\
2MASXJ07192718 & 109.863 & 54.229 & 0.067 & X & X & X &  & X \\
2MASXJ08374557 & 129.440 & 49.478 & 0.052 & X & X & X & X & X \\
2MASXJ09591230 & 149.801 & -9.003 & 0.033 & X & X & X &  & X \\
2MASXJ10525434 & 163.226 & 23.598 & 0.060 &  & X & X &  & X \\
2MASXJ11123493 & 168.145 & 12.072 & 0.046 & X & X & X &  &  \\
2MASXJ11500404 & 177.517 & 21.280 & 0.026 & X & X & X &  &  \\
2MASXJ12095669 & 182.486 & 47.096 & 0.031 &  & X & X &  & X \\
2MASXJ12385810 & 189.742 & 11.131 & 0.060 & X & X & X &  & X \\
2MASXJ15024995 & 225.708 & 48.784 & 0.026 &  & X & X &  & X \\
2MASXJ15393305 & 234.888 & 32.094 & 0.054 & X & X & X &  & X \\
2MASXJ15570268 & 239.261 & 37.417 & 0.031 & X & X & X & X & X \\
2MASXJ16065563 & 241.732 & 3.001 & 0.042 &  & X & X &  & X \\
2MASXJ16152860 & 243.869 & 19.226 & 0.033 & X & X & X & X & X \\
2MASXJ16301506 & 247.563 & 5.931 & 0.052 & X & X & X & X & X \\
2MASXJ17100856 & 257.536 & 74.729 & 0.042 & X & X & X & X & X \\
2MASXJ18242915 & 276.122 & 52.444 & 0.030 & X & X & X &  & X \\
2MASXJ21352164 & 323.840 & 26.935 & 0.067 & X & X & X &  & X \\
2MASXJ23024668 & 345.694 & 8.805 & 0.048 & X & X & X & X & X \\
2MFGC13321 & 249.372 & 40.880 & 0.026 & X & X & X &  & X \\
ANON. & 139.042 & 1.592 & 0.070 &  &  & X &  & X \\
ARP143 & 116.723 & 39.019 & 0.013 &  &  & X & X & X \\
ARP70 & 20.868 & 30.784 & 0.035 &  &  & X & X & X \\
CGCG004-035 & 127.075 & 0.289 & 0.030 & X & X & X & X & X \\
CGCG008-023 & 150.299 & 0.329 & 0.035 & X & X & X & X & X \\
CGCG042-196 & 189.959 & 3.797 & 0.040 & X & X & X &  & X \\
CGCG047-117 & 219.211 & 6.139 & 0.059 & X & X & X & X & X \\
CGCG064-017 & 149.812 & 12.988 & 0.034 & X & X & X &  & X \\
CGCG092-024 & 144.967 & 16.918 & 0.048 & X & X & X &  & X \\
CGCG107-031 & 235.995 & 19.212 & 0.024 & X & X & X & X & X \\
CGCG207-042 & 122.931 & 41.555 & 0.032 & X & X & X & X & X \\
CGCG229-009 & 284.514 & 43.936 & 0.028 & X & X & X &  & X \\
CGCG229-010 & 284.669 & 43.468 & 0.029 & X & X & X &  & X \\
CGCG308-009 & 92.127 & 64.724 & 0.014 & X & X & X & X & X \\
CGCG476117 & 355.660 & 27.092 & 0.025 & X & X & X & X & X \\
FGC175A & 191.603 & 11.950 & 0.046 & X & X & X & X & X \\
GALEXASCJ012052 & 20.220 & 3.340 & 0.034 & X & X & X & X & X \\
GALEXASCJ161311 & 243.299 & 1.592 & 0.033 & X & X & X &  & X \\
GALEXASCJ234457 & 356.240 & 3.394 & 0.052 & X & X & X & X & X \\
IC0208 & 32.116 & 6.395 & 0.012 & X & X & X & X & X \\
IC0391 & 74.338 & 78.189 & 0.005 & X & X & X &  & X \\
IC0701 & 172.753 & 20.469 & 0.020 & X & X & X & X & X \\
IC0758 & 181.050 & 62.505 & 0.004 & X & X & X & X & X \\
IC1277 & 272.614 & 31.003 & 0.024 & X & X & X &  &  \\
IC1481 & 349.855 & 5.906 & 0.020 & X & X & X & X & X \\
IC1890 & 47.494 & 19.208 & 0.034 & X & X & X &  & X \\
IC2373 & 126.704 & 20.365 & 0.025 & X & X & X & X & X \\
IC2481 & 141.870 & 3.930 & 0.018 & X & X & X & X & X \\
IC3918 & 194.223 & 22.374 & 0.022 & X & X & X & X & X \\
IC4526 & 225.659 & 23.350 & 0.046 & X & X & X & X & X \\
IC4582 & 236.414 & 28.089 & 0.007 & X & X & X & X & X \\
IZW45 & 193.276 & 36.823 & 0.028 &  &  & X &  & X \\
KUG0147+328B & 27.714 & 33.140 & 0.037 & X & X & X & X & X \\
KUG0210-078 & 33.316 & -7.662 & 0.016 & X & X & X & X & X \\
LEDA1709570 & 12.574 & 24.532 & 0.033 & X & X & X &  & X \\
M82 & 148.970 & -69.679 & 0.001 & X & X & X &  & X \\
MCG+02-58-008 & 341.552 & 10.557 & 0.039 &  & X & X &  & X \\
MCG+03-30-051 & 175.602 & 20.119 & 0.020 & X & X & X &  &  \\
MCG+03-30-38 & 243.299 & 1.592 & 0.011 & X & X & X &  & X \\
MCG+05-30-111 & 193.068 & 27.533 & 0.018 &  & X & X &  & X \\
MCG+07-05-39 & 35.146 & 41.574 & 0.022 & X & X & X &  & X \\
MCG+08-01-03 & 358.048 & 47.395 & 0.018 & X & X & X &  & X \\
MCG+08-10-07 & 82.186 & 49.883 & 0.023 & X & X & X &  & X \\
MCG+08-19-17 & 154.742 & 46.454 & 0.030 & X & X & X &  & X \\
MCG+08-36-16 & 300.708 & 49.320 & 0.024 & X & X & X &  & X \\
MCG+09-22-53 & 200.635 & 54.818 & 0.012 &  & X & X &  & X \\
MCG+11-08-25 & 93.955 & 66.839 & 0.014 & X & X & X &  & X \\
MCG+11-10-34 & 117.892 & 63.928 & 0.025 & X & X & X &  & X \\
MCG-01-09-006 & 47.201 & -7.041 & 0.029 & X & X & X & X & X \\
MCG-01-10-019 & 49.133 & -0.468 & 0.018 & X & X & X & X & X \\
MCG-01-33-12 & 192.256 & -9.457 & 0.013 & X & X & X & X & X \\
MCG-01-54-016 & 321.499 & -3.810 & 0.010 & X & X & X & X & X \\
MCG-02-02-086 & 10.460 & -9.303 & 0.056 & X & X & X & X & X \\
NGC0105 & 6.319 & 12.889 & 0.018 & X & X & X & X & X \\
NGC0214 & 10.367 & 25.499 & 0.015 & X & X & X & X & X \\
NGC0224 & 10.685 & 41.269 & 0.035 & X & X & X &  &  \\
NGC0309 & 14.178 & -9.914 & 0.019 & X & X & X & X & X \\
NGC0495 & 20.733 & 33.472 & 0.014 & X & X & X &  & X \\
NGC0523 & 21.337 & 34.025 & 0.016 & X & X & X & X & X \\
NGC0628 & 24.174 & 15.784 & 0.002 & X & X & X &  & X \\
NGC0691 & 27.674 & 21.760 & 0.009 & X & X & X & X & X \\
NGC0716 & 28.249 & 12.708 & 0.015 & X & X & X & X & X \\
NGC0774 & 29.895 & 14.008 & 0.015 & X & X & X & X & X \\
NGC0776 & 29.977 & 23.644 & 0.016 & X & X & X & X & X \\
NGC0890 & 35.504 & 33.266 & 0.013 & X & X & X &  & X \\
NGC0932 & 36.978 & 20.332 & 0.014 & X & X & X & X & X \\
NGC0938 & 37.140 & 20.284 & 0.014 & X & X & X & X & X \\
NGC0976 & 38.500 & 20.977 & 0.014 & X & X & X & X & X \\
NGC0991 & 38.886 & -7.154 & 0.005 & X & X & X & X & X \\
NGC1056 & 40.701 & 28.574 & 0.005 &  & X & X &  & X \\
NGC1058 & 40.875 & 37.341 & 0.002 & X & X & X &  & X \\
NGC1060 & 40.813 & 32.425 & 0.017 & X & X & X & X & X \\
NGC1070 & 40.843 & 4.968 & 0.014 & X & X & X & X & X \\
NGC1093 & 42.067 & 34.420 & 0.018 & X & X & X & X & X \\
NGC1142 & 43.801 & -0.184 & 0.029 & X & X & X & X & X \\
NGC1259 & 49.322 & 41.386 & 0.019 & X & X & X & X & X \\
NGC1590 & 67.793 & 7.631 & 0.013 & X & X & X &  & X \\
NGC1637 & 70.367 & -2.858 & 0.002 &  & X & X &  & X \\
NGC1667 & 72.155 & -6.320 & 0.015 & X & X & X & X & X \\
NGC2276A & 111.810 & 85.755 & 0.008 & X & X & X &  & X \\
NGC2276E & 111.810 & 85.755 & 0.008 & X & X & X &  & X \\
NGC2276F & 111.810 & 85.755 & 0.008 & X & X & X &  & X \\
NGC2315 & 105.638 & 50.591 & 0.021 & X & X & X &  & X \\
NGC2320 & 106.425 & 50.581 & 0.020 & X & X & X &  & X \\
NGC2333 & 107.089 & 35.170 & 0.016 & X & X & X &  & X \\
NGC2347 & 109.015 & 64.709 & 0.015 & X & X & X &  & X \\
NGC2431 & 116.306 & 53.075 & 0.019 & X & X & X &  & X \\
NGC2526 & 121.744 & 8.004 & 0.015 & X & X & X &  & X \\
NGC2554 & 124.473 & 23.472 & 0.014 & X & X & X & X & X \\
NGC2565 & 124.951 & 22.031 & 0.012 & X & X & X & X & X \\
NGC2577 & 125.681 & 22.553 & 0.007 & X & X & X &  & X \\
NGC2595 & 126.925 & 21.479 & 0.014 & X & X & X & X & X \\
NGC2596 & 126.860 & 17.284 & 0.020 & X & X & X & X & X \\
NGC2604 & 128.346 & 29.539 & 0.007 & X & X & X &  & X \\
NGC2618 & 128.973 & 0.707 & 0.013 & X & X & X & X & X \\
NGC2623 & 129.600 & 25.755 & 0.019 & X & X & X & X & X \\
NGC2639 & 130.909 & 50.206 & 0.011 & X & X & X & X & X \\
NGC2691 & 133.693 & 39.539 & 0.013 & X & X & X & X & X \\
NGC2748 & 138.429 & 76.475 & 0.005 & X & X & X &  & X \\
NGC2765 & 136.903 & 3.393 & 0.013 & X & X & X & X & X \\
NGC2771 & 137.665 & 50.380 & 0.017 & X & X & X & X & X \\
NGC2789 & 138.749 & 29.730 & 0.021 & X & X & X & X & X \\
NGC2906 & 143.026 & 8.442 & 0.007 & X & X & X & X & X \\
NGC2916 & 143.740 & 21.705 & 0.012 & X & X & X & X & X \\
NGC2926 & 144.379 & 32.841 & 0.015 & X & X & X & X & X \\
NGC3057 & 151.414 & 80.286 & 0.005 & X & X & X & X & X \\
NGC3158 & 153.460 & 38.765 & 0.023 & X & X & X & X & X \\
NGC3184 & 154.570 & 41.424 & 0.002 & X & X & X &  & X \\
NGC3310 & 159.691 & 53.503 & 0.003 & X & X & X & X & X \\
NGC3323 & 159.913 & 25.323 & 0.017 & X & X & X & X & X \\
NGC3451 & 163.587 & 27.240 & 0.004 & X & X & X & X & X \\
NGC3499 & 165.796 & 56.222 & 0.005 &  & X & X &  & X \\
NGC3655 & 170.728 & 16.590 & 0.005 & X & X & X & X & X \\
NGC3687 & 172.003 & 29.511 & 0.008 & X & X & X & X & X \\
NGC3774 & 174.626 & -8.976 & 0.021 &  & X & X &  &  \\
NGC3811 & 175.319 & 47.691 & 0.010 & X & X & X & X & X \\
NGC3847 & 176.058 & 33.515 & 0.032 & X & X & X &  & X \\
NGC3861 & 176.266 & 19.974 & 0.017 & X & X & X & X & X \\
NGC3905 & 177.270 & -9.730 & 0.019 & X & X & X &  & X \\
NGC3913 & 177.662 & 55.354 & 0.003 &  & X & X &  & X \\
NGC3982 & 179.117 & 55.125 & 0.004 &  & X & X &  & X \\
NGC4070 & 181.047 & 20.410 & 0.025 & X & X & X & X & X \\
NGC4210 & 183.816 & 65.985 & 0.009 & X & X & X &  & X \\
NGC4384 & 186.300 & 54.506 & 0.008 & X & X & X & X & X \\
NGC4470 & 187.407 & 7.824 & 0.008 & X & X & X & X & X \\
NGC4644 & 190.678 & 55.146 & 0.017 &  & X & X &  & X \\
NGC4866 & 194.863 & 14.171 & 0.007 & X & X & X & X & X \\
NGC4874 & 194.899 & 27.959 & 0.024 & X & X & X & X & X \\
NGC4961 & 196.448 & 27.734 & 0.008 & X & X & X & X & X \\
NGC5000 & 197.448 & 28.907 & 0.019 & X & X & X & X & X \\
NGC5056 & 199.051 & 30.950 & 0.019 & X & X & X & X & X \\
NGC5157 & 201.820 & 32.031 & 0.024 & X & X & X & X & X \\
NGC5338 & 208.361 & 5.208 & 0.003 & X & X & X &  & X \\
NGC5339 & 208.501 & -7.931 & 0.009 & X & X & X & X & X \\
NGC5378 & 209.213 & 37.797 & 0.010 & X & X & X & X & X \\
NGC5406 & 210.084 & 38.915 & 0.017 & X & X & X & X & X \\
NGC5410 & 210.228 & 40.989 & 0.012 & X & X & X &  & X \\
NGC5421 & 210.425 & 33.822 & 0.025 & X & X & X & X & X \\
NGC5425 & 210.199 & 48.444 & 0.007 & X & X & X &  & X \\
NGC5426 & 210.854 & -6.069 & 0.009 & X & X & X &  & X \\
NGC5468 & 211.645 & -5.453 & 0.009 & X & X & X &  & X \\
NGC5480 & 211.590 & 50.725 & 0.006 &  & X & X &  & X \\
NGC5525 & 213.913 & 14.283 & 0.019 & X & X & X & X & X \\
NGC5557 & 214.607 & 36.494 & 0.011 & X & X & X & X & X \\
NGC5559 & 214.803 & 24.799 & 0.017 & X & X & X & X & X \\
NGC5587 & 215.545 & 13.918 & 0.008 & X & X & X & X & X \\
NGC5611 & 216.020 & 33.047 & 0.007 & X & X & X &  & X \\
NGC5630 & 216.903 & 41.258 & 0.009 & X & X & X & X & X \\
NGC5668 & 218.351 & 4.450 & 0.005 & X & X & X & X & X \\
NGC5682 & 218.687 & 48.670 & 0.008 & X & X & X & X & X \\
NGC5714 & 219.548 & 46.638 & 0.007 & X & X & X & X & X \\
NGC5732 & 220.162 & 38.638 & 0.013 & X & X & X & X & X \\
NGC5735 & 220.639 & 28.726 & 0.012 & X & X & X & X & X \\
NGC5772 & 222.912 & 40.599 & 0.016 & X & X & X & X & X \\
NGC5829 & 225.675 & 23.334 & 0.019 & X & X & X & X & X \\
NGC5837 & 226.169 & 12.633 & 0.029 & X & X & X & X & X \\
NGC5888 & 228.281 & 41.265 & 0.029 & X & X & X & X & X \\
NGC5910 & 229.853 & 20.896 & 0.041 & X & X & X &  & X \\
NGC5980 & 235.377 & 15.788 & 0.014 & X & X & X & X & X \\
NGC5996 & 236.745 & 17.884 & 0.011 & X & X & X & X & X \\
NGC6063 & 241.804 & 7.979 & 0.010 & X & X & X & X & X \\
NGC6146 & 246.293 & 40.893 & 0.029 & X & X & X &  & X \\
NGC6166 & 247.160 & 39.552 & 0.031 & X & X & X & X & X \\
NGC6173 & 247.437 & 40.812 & 0.029 & X & X & X &  & X \\
NGC6186 & 248.606 & 21.541 & 0.010 & X & X & X &  & X \\
NGC6261 & 254.127 & 27.978 & 0.035 & X & X & X & X & X \\
NGC6373 & 261.034 & 58.995 & 0.011 & X & X & X & X & X \\
NGC6643 & 274.943 & 74.568 & 0.005 & X & X & X &  & X \\
NGC6786 & 287.725 & 73.410 & 0.025 & X & X & X &  & X \\
NGC6946 & 308.718 & 60.154 & 0.000 & X & X & X &  & X \\
NGC6962 & 311.829 & 0.321 & 0.014 & X & X & X & X & X \\
NGC7033 & 317.401 & 15.125 & 0.030 & X & X & X &  & X \\
NGC7042 & 318.441 & 13.575 & 0.017 & X & X & X &  & X \\
NGC7047 & 319.115 & -0.826 & 0.019 & X & X & X & X & X \\
NGC7222 & 332.716 & 2.106 & 0.041 & X & X & X & X & X \\
NGC7253 & 334.875 & 29.388 & 0.016 & X & X & X & X & X \\
NGC7311 & 338.528 & 5.570 & 0.015 & X & X & X & X & X \\
NGC7319 & 339.015 & 33.976 & 0.023 & X & X & X & X & X \\
NGC7321 & 339.117 & 21.622 & 0.024 & X & X & X & X & X \\
NGC7364 & 341.102 & -0.162 & 0.016 & X & X & X & X & X \\
NGC7461 & 345.451 & 15.582 & 0.014 &  & X & X &  & X \\
NGC7469 & 345.815 & 8.874 & 0.016 & X & X & X & X & X \\
NGC7489 & 346.886 & 22.998 & 0.021 & X & X & X & X & X \\
NGC7503 & 347.676 & 7.568 & 0.044 & X & X & X &  & X \\
NGC7619 & 350.061 & 8.206 & 0.013 & X & X & X & X & X \\
NGC7653 & 351.206 & 15.276 & 0.014 & X & X & X &  & X \\
NGC7691 & 353.102 & 15.848 & 0.013 & X & X & X & X & X \\
NGC7771 & 357.853 & 20.112 & 0.014 & X & X & X & X & X \\
NGC7803 & 0.333 & 13.111 & 0.018 & X & X & X & X & X \\
PGC0010652 & 42.221 & 53.037 & 0.017 & X & X & X &  & X \\
PGC0014370 & 60.820 & 71.720 & 0.015 &  & X & X &  & X \\
PGC0035860 & 173.963 & 34.282 & 0.021 & X & X & X & X & X \\
PGC0213858 & 173.654 & 54.891 & 0.019 & X & X & X &  & X \\
PGC063016 & 289.321 & 33.425 & 0.015 &  & X & X &  & X \\
PGC067911 & 330.684 & 31.696 & 0.016 & X & X & X &  & X \\
PGC10738 & 42.537 & 12.844 & 0.034 & X & X & X &  & X \\
PGC11179 & 44.390 & 5.977 & 0.023 & X & X & X & X & X \\
PGC1481751 & 30.420 & 15.331 & 0.033 & X & X & X &  & X \\
PGC213672 & 152.332 & 14.991 & 0.030 & X & X & X &  & X \\
PGC3086846 & 146.282 & 58.669 & 0.030 & X & X & X &  & X \\
PGC34730 & 170.161 & -3.546 & 0.025 &  & X & X &  & X \\
PGC37426 & 178.877 & 11.924 & 0.021 & X & X & X & X & X \\
PGC74050 & 29.566 & 36.348 & 0.016 & X & X & X &  & X \\
SDSSJ004750 & 11.962 & 31.823 & 0.087 & X & X & X &  & X \\
SDSSJ02595365 & 44.974 & 1.160 & 0.073 &  & X & X &  & X \\
SDSSJ083516 & 128.818 & 48.317 & 0.043 & X & X & X & X & X \\
SDSSJ08535700 & 133.488 & 17.328 & 0.067 & X & X & X &  & X \\
SDSSJ120951251947165 & 182.464 & 19.788 & 0.043 & X & X & X & X & X \\
SDSSJ161812 & 244.552 & 36.484 & 0.028 & X & X & X & X & X \\
SDSSJ170413 & 256.055 & 17.816 & 0.080 & X & X & X &  & X \\
UGC00005 & 0.774 & -1.914 & 0.024 & X & X & X & X & X \\
UGC00040 & 1.452 & 27.449 & 0.025 & X & X & X & X & X \\
UGC00139 & 3.633 & -0.738 & 0.013 & X & X & X & X & X \\
UGC00148 & 3.964 & 16.090 & 0.014 &  & X & X &  & X \\
UGC01087 & 22.861 & 14.278 & 0.015 &  & X & X &  & X \\
UGC02134 & 39.716 & 27.847 & 0.015 & X & X & X &  & X \\
UGC02175 & 40.569 & 42.393 & 0.014 & X & X & X &  & X \\
UGC02308 & 42.551 & 47.054 & 0.028 & X & X & X &  & X \\
UGC02628 & 49.133 & -0.468 & 0.023 & X & X & X & X & X \\
UGC02756 & 52.396 & 40.869 & 0.017 &  & X & X &  & X \\
UGC02829 & 55.462 & 8.160 & 0.021 & X & X & X & X & X \\
UGC02836 & 55.987 & 39.295 & 0.017 & X & X & X & X & X \\
UGC02912 & 59.889 & 42.617 & 0.018 & X & X & X &  & X \\
UGC02931 & 60.577 & 25.817 & 0.019 & X & X & X &  & X \\
UGC03108 & 69.618 & 44.037 & 0.013 & X & X & X &  & X \\
UGC03151 & 71.332 & 11.068 & 0.015 &  & X & X &  & X \\
UGC03312 & 82.168 & 22.114 & 0.019 & X & X & X &  & X \\
UGC03513 & 100.716 & 41.421 & 0.025 & X & X & X &  & X \\
UGC03552 & 102.464 & 28.371 & 0.016 & X & X & X & X & X \\
UGC03555 & 102.499 & 25.634 & 0.016 & X & X & X &  & X \\
UGC03611 & 104.299 & 20.437 & 0.017 &  & X & X &  & X \\
UGC03627 & 105.271 & 51.270 & 0.021 & X & X & X &  & X \\
UGC03770 & 108.873 & 23.426 & 0.021 & X & X & X &  & X \\
UGC03843 & 111.432 & 20.102 & 0.018 & X & X & X &  & X \\
UGC03944 & 114.652 & 37.634 & 0.013 & X & X & X & X & X \\
UGC04008 & 116.653 & 44.798 & 0.031 & X & X & X & X & X \\
UGC04036 & 117.978 & 73.016 & 0.012 & X & X & X &  & X \\
UGC04107 & 119.258 & 49.567 & 0.012 &  & X & X &  & X \\
UGC04132 & 119.804 & 32.915 & 0.017 & X & X & X & X & X \\
UGC04179 & 120.524 & 0.809 & 0.019 & X & X & X & X & X \\
UGC04195 & 121.279 & 66.783 & 0.016 & X & X & X & X & X \\
UGC04308 & 124.358 & 21.685 & 0.012 & X & X & X & X & X \\
UGC04310 & 124.315 & 1.206 & 0.015 & X & X & X & X & X \\
UGC04414 & 126.775 & 21.645 & 0.025 & X & X & X & X & X \\
UGC04423 & 127.722 & 74.687 & 0.012 &  & X & X &  & X \\
UGC04455 & 127.887 & -1.198 & 0.031 & X & X & X & X & X \\
UGC04461 & 128.344 & 52.532 & 0.017 & X & X & X & X & X \\
UGC04468 & 128.378 & 41.525 & 0.025 & X & X & X &  & X \\
UGC04981 & 141.008 & 68.562 & 0.013 & X & X & X &  & X \\
UGC05100 & 143.661 & 5.841 & 0.018 & X & X & X & X & X \\
UGC05129 & 144.492 & 25.495 & 0.014 & X & X & X & X & X \\
UGC05392 & 150.399 & 21.608 & 0.021 &  & X & X &  & X \\
UGC05520 & 153.752 & 65.140 & 0.011 &  & X & X &  & X \\
UGC05695 & 157.445 & 13.018 & 0.010 & X & X & X & X & X \\
UGC06036 & 163.980 & 36.862 & 0.022 & X & X & X & X & X \\
UGC06483 & 172.260 & 17.232 & 0.013 & X & X & X &  &  \\
UGC06517 & 173.010 & 36.698 & 0.008 & X & X & X & X & X \\
UGC06609 & 174.623 & 20.528 & 0.026 & X & X & X &  &  \\
UGC07170 & 182.654 & 18.828 & 0.008 & X & X & X &  &  \\
UGC07228 & 183.403 & 46.494 & 0.025 & X & X & X & X & X \\
UGC08250 & 197.584 & 32.483 & 0.018 & X & X & X & X & X \\
UGC08472 & 202.307 & 11.276 & 0.022 & X & X & X &  & X \\
UGC08503 & 202.687 & 32.761 & 0.016 & X & X & X & X & X \\
UGC08733 & 207.162 & 43.412 & 0.008 & X & X & X & X & X \\
UGC08932 & 210.235 & 41.005 & 0.012 & X & X & X &  & X \\
UGC09165 & 214.699 & 24.940 & 0.018 & X & X & X & X & X \\
UGC09356 & 218.223 & 11.595 & 0.007 & X & X & X & X & X \\
UGC09391 & 218.654 & 59.338 & 0.006 & X & X & X &  &  \\
UGC09629 & 224.297 & 52.346 & 0.026 & X & X & X &  &  \\
UGC09842 & 231.274 & 37.960 & 0.030 & X & X & X & X & X \\
UGC10064 & 237.805 & 25.702 & 0.022 & X & X & X & X & X \\
UGC10097 & 238.930 & 47.867 & 0.020 &  & X & X &  & X \\
UGC10123 & 239.762 & 51.305 & 0.013 & X & X & X &  & X \\
UGC10331 & 244.338 & 59.320 & 0.015 & X & X & X & X & X \\
UGC10414 & 247.447 & 8.644 & 0.033 & X & X & X &  & X \\
UGC1071 & 22.449 & -1.984 & 0.020 & X & X & X & X & X \\
UGC11064 & 269.421 & 27.835 & 0.023 & X & X & X &  & X \\
UGC11162 & 273.253 & 29.696 & 0.015 & X & X & X &  & X \\
UGC11241 & 276.708 & 51.139 & 0.033 &  & X & X &  &  \\
UGC11260 & 277.606 & 34.103 & 0.021 & X & X & X &  & X \\
UGC11723 & 320.073 & -1.684 & 0.016 & X & X & X & X & X \\
UGC11758 & 322.740 & 13.986 & 0.029 & X & X & X &  & X \\
UGC11922 & 332.226 & 40.349 & 0.024 & X & X & X &  & X \\
UGC11975 & 334.332 & 35.571 & 0.021 & X & X & X &  & X \\
UGC12157 & 340.465 & 34.968 & 0.033 & X & X & X &  & X \\
UGC12809 & 357.763 & 46.724 & 0.046 & X & X & X &  & X \\
UGC12810 & 357.776 & 1.057 & 0.027 & X & X & X & X & X \\
UGC12850 & 359.026 & 29.378 & 0.023 & X & X & X &  & X \\
UGC2164 & 40.289 & 43.683 & 0.023 & X & X & X &  & X \\
UGC3236 & 75.888 & 6.657 & 0.028 & X & X & X &  & X \\
UGC6837 & 177.969 & 18.546 & 0.020 & X & X & X & X & X
\enddata
\end{deluxetable}


==> global_photometry_2mass_full.tex <==
\begin{deluxetable}{lrrrrrr}
\tablecaption{In-house global photometry 2MASS.  Only 2MASS photometry with SDSS coverage was measured. Given as AB magnitudes. -99 marks negative flux. } \rotate \label{table:global_photometry_2mass}
\tablehead{\colhead{Galaxy} & \colhead{$m_H$} & \colhead{$\sigma_{m_H}$} & \colhead{$m_J$} & \colhead{$\sigma_{m_J}$} & \colhead{$m_K$} & \colhead{$\sigma_{m_K}$}}
\startdata
2MASSJ00164451 & 15.485 & 0.397 & 16.047 & 0.451 & 16.439 & 1.304 \\
2MASSJ00235669 & 15.755 & 0.479 & 16.203 & 0.475 & 18.210 & 5.562 \\
2MASSJ23243021 & 15.358 & 0.324 & 15.465 & 0.268 & 15.180 & 0.404 \\
2MASXJ00234829 & 13.329 & 0.171 & 14.607 & 0.326 & 14.105 & 0.417 \\
2MASXJ01144386 & -99.000 & -99.000 & 14.672 & 0.377 & 14.144 & 0.455 \\
2MASXJ01403375 & 13.856 & 0.208 & 14.157 & 0.182 & 13.793 & 0.242 \\
2MASXJ02305208 & 13.160 & 0.100 & 13.805 & 0.104 & 13.574 & 0.134 \\
2MASXJ08374557 & 14.847 & 0.462 & 15.332 & 0.506 & 14.678 & 0.456 \\
2MASXJ10525434 & -99.000 & -99.000 & 15.940 & 0.948 & -99.000 & -99.000 \\
2MASXJ11123493 & 14.657 & 0.504 & 14.719 & 0.399 & 14.487 & 0.567 \\
2MASXJ11500404 & 12.939 & 0.120 & 13.699 & 0.097 & 13.465 & 0.150 \\
2MASXJ12095669 & 14.019 & 0.268 & 14.034 & 0.156 & 14.034 & 0.250 \\
2MASXJ12385810 & 16.121 & 2.423 & 15.263 & 0.731 & 14.925 & 0.922 \\
2MASXJ15024995 & 14.778 & 0.570 & 15.113 & 0.463 & 14.607 & 0.453 \\
2MASXJ15393305 & 12.818 & 0.127 & 13.347 & 0.129 & 13.106 & 0.165 \\
2MASXJ15570268 & 14.630 & 0.406 & 14.387 & 0.203 & 14.981 & 0.547 \\
2MASXJ16065563 & 13.338 & 0.244 & 13.982 & 0.316 & 13.817 & 0.426 \\
2MASXJ16152860 & 13.842 & 0.192 & 14.678 & 0.251 & 14.398 & 0.321 \\
2MASXJ16301506 & 13.701 & 0.179 & 13.994 & 0.158 & 13.769 & 0.232 \\
2MASXJ17100856 & 14.163 & 0.183 & 14.317 & 0.139 & 13.955 & 0.189 \\
2MASXJ21352164 & 13.649 & 0.231 & 13.797 & 0.180 & 14.021 & 0.288 \\
2MASXJ22532475 & 14.868 & 0.777 & 13.796 & 0.187 & 14.147 & 0.419 \\
2MASXJ23024668 & 13.672 & 0.143 & 14.053 & 0.097 & 14.050 & 0.158 \\
ARP143 & 11.349 & 0.082 & 10.893 & 0.035 & 11.070 & 0.066 \\
ARP70 & 12.872 & 0.270 & 12.415 & 0.098 & 12.783 & 0.194 \\
CGCG004-035 & 11.905 & 0.092 & 12.186 & 0.086 & 12.360 & 0.159 \\
CGCG008-023 & 14.030 & 0.403 & 13.985 & 0.276 & 13.637 & 0.333 \\
CGCG042-196 & 13.199 & 0.172 & 14.169 & 0.297 & 13.852 & 0.407 \\
CGCG047-117 & 13.286 & 0.187 & 13.608 & 0.183 & 13.785 & 0.397 \\
CGCG064-017 & 13.676 & 0.211 & 14.189 & 0.180 & 14.149 & 0.299 \\
CGCG092-024 & 15.302 & 2.143 & 13.222 & 0.202 & 13.430 & 0.376 \\
CGCG107-031 & 12.783 & 0.169 & 12.801 & 0.107 & 12.529 & 0.129 \\
CGCG207-042 & 12.594 & 0.118 & 13.621 & 0.174 & 13.253 & 0.201 \\
CGCG308-009 & 12.405 & 0.100 & 12.062 & 0.044 & 12.652 & 0.133 \\
CGCG476117 & 15.115 & 1.331 & 13.384 & 0.164 & 13.633 & 0.281 \\
FGC175A & 14.581 & 0.441 & 15.570 & 0.818 & 14.506 & 0.530 \\
GALEXASCJ012052 & 13.455 & 0.383 & 15.400 & 0.882 & 14.669 & 0.782 \\
GALEXASCJ234457 & 14.839 & 0.681 & 15.086 & 0.443 & 14.112 & 0.292 \\
IC0208 & 13.321 & 0.466 & 12.291 & 0.117 & 12.944 & 0.401 \\
IC0701 & 12.959 & 0.217 & 13.150 & 0.158 & 13.624 & 0.365 \\
IC0758 & 10.799 & 0.067 & 12.159 & 0.134 & 11.289 & 0.111 \\
IC1481 & 12.204 & 0.087 & 11.767 & 0.041 & 12.204 & 0.090 \\
IC1890 & 11.319 & 0.041 & 11.499 & 0.034 & 11.485 & 0.060 \\
IC2373 & 13.558 & 0.522 & 15.144 & 1.080 & 13.679 & 0.471 \\
IC2481 & 12.356 & 0.133 & 12.948 & 0.166 & 12.767 & 0.238 \\
IC3918 & 15.399 & 1.063 & 14.609 & 0.355 & 15.391 & 1.206 \\
IC4526 & 13.957 & 0.373 & 13.565 & 0.159 & 14.167 & 0.517 \\
IC4582 & 13.657 & 0.499 & 12.976 & 0.145 & 13.374 & 0.313 \\
IZW45 & 12.924 & 0.107 & 13.106 & 0.085 & 12.966 & 0.115 \\
KUG0147+328B & 16.204 & 1.993 & 15.904 & 0.993 & -99.000 & -99.000 \\
KUG0210-078 & 11.180 & 0.077 & 11.561 & 0.055 & 11.651 & 0.098 \\
LEDA1709570 & -99.000 & -99.000 & 15.160 & 0.545 & 15.924 & 1.806 \\
MCG+02-58-008 & 11.203 & 0.067 & 12.111 & 0.060 & 11.803 & 0.079 \\
MCG+03-30-051 & 12.787 & 0.159 & 12.786 & 0.103 & 12.887 & 0.206 \\
MCG+08-19-17 & 14.676 & 0.461 & 14.449 & 0.253 & 14.332 & 0.367 \\
MCG+09-22-53 & 12.793 & 0.095 & 13.121 & 0.092 & 13.304 & 0.169 \\
MCG-01-09-006 & -99.000 & -99.000 & 12.959 & 0.191 & 13.781 & 0.718 \\
MCG-01-10-019 & 12.873 & 0.243 & 12.779 & 0.134 & 12.721 & 0.240 \\
MCG-01-33-12 & 12.804 & 0.280 & 12.984 & 0.237 & 15.708 & 5.461 \\
MCG-01-54-016 & -99.000 & -99.000 & 15.100 & 1.080 & 13.687 & 0.483 \\
MCG-02-02-086 & 11.697 & 0.064 & 11.745 & 0.044 & 11.719 & 0.086 \\
NGC0105 & 12.662 & 0.103 & 12.481 & 0.048 & 12.539 & 0.085 \\
NGC0214 & 10.265 & 0.030 & 10.874 & 0.027 & 11.247 & 0.066 \\
NGC0309 & 10.919 & 0.045 & 11.039 & 0.035 & 11.129 & 0.068 \\
NGC0495 & 14.255 & 1.113 & 11.890 & 0.071 & 12.157 & 0.120 \\
NGC0523 & 11.502 & 0.064 & 11.481 & 0.038 & 11.552 & 0.065 \\
NGC0691 & 9.329 & 0.011 & 9.368 & 0.007 & 9.761 & 0.019 \\
NGC0716 & 10.888 & 0.038 & 11.601 & 0.055 & 11.239 & 0.077 \\
NGC0774 & 10.816 & 0.039 & 11.369 & 0.040 & 11.431 & 0.082 \\
NGC0776 & 11.107 & 0.062 & 11.280 & 0.051 & 11.503 & 0.109 \\
NGC0932 & 10.488 & 0.031 & 10.740 & 0.027 & 10.948 & 0.057 \\
NGC0938 & 11.198 & 0.055 & 11.217 & 0.032 & 11.466 & 0.068 \\
NGC0976 & 10.835 & 0.043 & 10.940 & 0.031 & 10.896 & 0.048 \\
NGC0991 & 11.071 & 0.069 & 11.474 & 0.065 & 11.157 & 0.094 \\
NGC1056 & 10.616 & 0.034 & 10.789 & 0.023 & 10.853 & 0.038 \\
NGC1060 & 9.644 & 0.018 & 9.846 & 0.014 & 9.871 & 0.021 \\
NGC1070 & 9.986 & 0.027 & 10.316 & 0.022 & 10.271 & 0.034 \\
NGC1093 & 11.013 & 0.052 & 11.965 & 0.065 & 11.844 & 0.095 \\
NGC1142 & 10.470 & 0.024 & 10.768 & 0.019 & 10.737 & 0.031 \\
NGC1259 & 11.671 & 0.068 & 12.060 & 0.061 & 11.964 & 0.085 \\
NGC1590 & 12.471 & 0.121 & 12.114 & 0.054 & 12.149 & 0.078 \\
NGC1667 & 9.939 & 0.030 & 10.521 & 0.030 & 10.317 & 0.043 \\
NGC2526 & 11.712 & 0.064 & 12.315 & 0.065 & 12.238 & 0.092 \\
NGC2554 & 10.256 & 0.026 & 10.406 & 0.019 & 10.539 & 0.033 \\
NGC2565 & 10.675 & 0.037 & 10.878 & 0.027 & 10.923 & 0.042 \\
NGC2577 & 10.636 & 0.030 & 10.744 & 0.020 & 10.788 & 0.031 \\
NGC2595 & -99.000 & -99.000 & 11.626 & 0.084 & -99.000 & -99.000 \\
NGC2596 & 11.276 & 0.061 & 12.015 & 0.076 & 11.768 & 0.106 \\
NGC2604 & 10.548 & 0.045 & 11.543 & 0.069 & 11.037 & 0.069 \\
NGC2618 & 11.468 & 0.128 & 11.124 & 0.066 & 11.358 & 0.128 \\
NGC2623 & -99.000 & -99.000 & 13.607 & 0.271 & -99.000 & -99.000 \\
NGC2639 & 10.099 & 0.019 & 10.267 & 0.016 & 10.256 & 0.025 \\
NGC2691 & 11.687 & 0.063 & 12.005 & 0.050 & 12.223 & 0.101 \\
NGC2765 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 \\
NGC2771 & 11.332 & 0.065 & 11.557 & 0.047 & 11.461 & 0.073 \\
NGC2789 & 11.160 & 0.052 & 11.578 & 0.050 & 11.501 & 0.066 \\
NGC2906 & 11.080 & 0.068 & 10.988 & 0.042 & 10.937 & 0.070 \\
NGC2916 & 10.870 & 0.056 & 11.045 & 0.043 & 10.973 & 0.062 \\
NGC2926 & -99.000 & -99.000 & 14.602 & 0.652 & 12.864 & 0.226 \\
NGC3057 & 12.620 & 0.218 & 12.946 & 0.166 & 12.948 & 0.244 \\
NGC3158 & 10.229 & 0.020 & 10.396 & 0.015 & 10.345 & 0.022 \\
NGC3310 & 10.102 & 0.028 & 10.169 & 0.017 & 10.357 & 0.030 \\
NGC3323 & 12.432 & 0.160 & 12.732 & 0.133 & 12.695 & 0.194 \\
NGC3451 & 11.489 & 0.056 & 11.947 & 0.059 & 11.732 & 0.085 \\
NGC3499 & 12.411 & 0.097 & 12.221 & 0.048 & 12.485 & 0.111 \\
NGC3655 & 10.407 & 0.034 & 10.596 & 0.025 & 10.635 & 0.038 \\
NGC3687 & 14.032 & 0.781 & 11.662 & 0.052 & 12.083 & 0.120 \\
NGC3811 & 11.195 & 0.069 & 11.353 & 0.042 & 11.513 & 0.094 \\
NGC3847 & 11.383 & 0.049 & 11.616 & 0.035 & 11.699 & 0.059 \\
NGC3861 & 11.412 & 0.066 & 11.645 & 0.061 & 11.792 & 0.107 \\
NGC3913 & 11.847 & 0.088 & 12.027 & 0.068 & 11.941 & 0.110 \\
NGC3982 & 10.434 & 0.036 & 10.615 & 0.027 & 10.795 & 0.051 \\
NGC4070 & 11.018 & 0.034 & 11.390 & 0.032 & 11.381 & 0.055 \\
NGC4210 & 10.901 & 0.076 & 11.398 & 0.073 & 11.430 & 0.125 \\
NGC4384 & 11.446 & 0.085 & 12.159 & 0.111 & 11.805 & 0.123 \\
NGC4470 & 11.952 & 0.178 & 11.801 & 0.098 & 11.973 & 0.188 \\
NGC4644 & 12.507 & 0.133 & 12.415 & 0.077 & 12.608 & 0.163 \\
NGC4866 & 9.399 & 0.016 & 9.629 & 0.011 & 9.605 & 0.019 \\
NGC4874 & 10.152 & 0.025 & 10.467 & 0.020 & 10.320 & 0.027 \\
NGC4961 & 11.173 & 0.062 & 12.252 & 0.099 & 12.115 & 0.132 \\
NGC5000 & 11.488 & 0.070 & 12.088 & 0.078 & 11.760 & 0.094 \\
NGC5056 & 9.094 & 0.015 & 10.846 & 0.025 & 10.228 & 0.025 \\
NGC5157 & 11.733 & 0.092 & 11.801 & 0.064 & 11.624 & 0.090 \\
NGC5338 & 11.971 & 0.120 & 11.957 & 0.091 & 12.352 & 0.235 \\
NGC5339 & 10.491 & 0.047 & 10.917 & 0.051 & 10.927 & 0.084 \\
NGC5378 & 11.286 & 0.061 & 11.382 & 0.046 & 11.503 & 0.089 \\
NGC5406 & 10.687 & 0.039 & 11.226 & 0.043 & 11.003 & 0.059 \\
NGC5410 & 11.988 & 0.106 & 13.020 & 0.169 & 12.274 & 0.155 \\
NGC5421 & 11.450 & 0.044 & 11.781 & 0.036 & 11.733 & 0.059 \\
NGC5425 & 12.766 & 0.180 & 12.776 & 0.137 & 13.212 & 0.333 \\
NGC5480 & 10.035 & 0.029 & 10.579 & 0.030 & 9.989 & 0.035 \\
NGC5525 & 11.010 & 0.043 & 11.256 & 0.034 & 11.206 & 0.049 \\
NGC5557 & 9.524 & 0.011 & 9.735 & 0.010 & 9.735 & 0.018 \\
NGC5559 & 11.792 & 0.065 & 12.085 & 0.062 & 12.000 & 0.087 \\
NGC5587 & 11.459 & 0.069 & 11.605 & 0.052 & 11.973 & 0.112 \\
NGC5611 & 11.494 & 0.047 & 11.472 & 0.030 & 11.562 & 0.057 \\
NGC5630 & 12.520 & 0.157 & 12.452 & 0.106 & 12.809 & 0.277 \\
NGC5668 & 10.026 & 0.046 & 10.709 & 0.042 & 10.986 & 0.091 \\
NGC5682 & 11.916 & 0.103 & 12.488 & 0.100 & 12.249 & 0.122 \\
NGC5714 & 11.466 & 0.085 & 12.049 & 0.087 & 12.247 & 0.162 \\
NGC5732 & -99.000 & -99.000 & 13.944 & 0.411 & 13.509 & 0.494 \\
NGC5735 & 11.362 & 0.081 & 11.952 & 0.090 & 12.007 & 0.165 \\
NGC5772 & 10.596 & 0.040 & 11.200 & 0.041 & 10.875 & 0.056 \\
NGC5829 & 14.186 & 0.964 & 12.457 & 0.118 & 14.537 & 1.480 \\
NGC5837 & 11.742 & 0.080 & 12.322 & 0.081 & 11.840 & 0.091 \\
NGC5888 & 11.658 & 0.081 & 11.760 & 0.061 & 11.613 & 0.098 \\
NGC5910 & 11.038 & 0.033 & 11.278 & 0.032 & 11.317 & 0.061 \\
NGC5980 & 11.118 & 0.058 & 11.286 & 0.043 & 11.262 & 0.072 \\
NGC5996 & 11.696 & 0.080 & 11.902 & 0.059 & 11.950 & 0.093 \\
NGC6063 & 12.834 & 0.390 & 12.040 & 0.125 & 11.983 & 0.220 \\
NGC6146 & 10.979 & 0.033 & 11.101 & 0.027 & 11.208 & 0.051 \\
NGC6166 & 10.798 & 0.050 & 10.789 & 0.030 & 10.682 & 0.046 \\
NGC6173 & 10.275 & 0.039 & 10.725 & 0.028 & 10.485 & 0.045 \\
NGC6186 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 \\
NGC6261 & 11.696 & 0.067 & 12.044 & 0.054 & 12.052 & 0.082 \\
NGC6373 & 11.977 & 0.152 & 13.312 & 0.319 & 12.724 & 0.288 \\
NGC6962 & 10.310 & 0.033 & 10.332 & 0.021 & 10.438 & 0.034 \\
NGC7047 & 11.617 & 0.125 & 11.805 & 0.078 & 12.178 & 0.184 \\
NGC7222 & 11.566 & 0.083 & 12.117 & 0.086 & 12.011 & 0.137 \\
NGC7253 & 11.130 & 0.110 & 11.670 & 0.066 & 11.505 & 0.112 \\
NGC7311 & 10.563 & 0.028 & 10.681 & 0.022 & 10.674 & 0.032 \\
NGC7319 & 11.275 & 0.044 & 11.678 & 0.043 & 11.720 & 0.077 \\
NGC7321 & 11.243 & 0.056 & 11.559 & 0.059 & 11.373 & 0.095 \\
NGC7364 & 11.746 & 0.105 & 11.278 & 0.033 & 11.383 & 0.066 \\
NGC7461 & 11.350 & 0.045 & 11.639 & 0.040 & 11.390 & 0.060 \\
NGC7469 & 10.670 & 0.032 & 10.933 & 0.026 & 10.782 & 0.037 \\
NGC7489 & -99.000 & -99.000 & 12.124 & 0.104 & 12.329 & 0.215 \\
NGC7503 & 11.720 & 0.073 & 11.851 & 0.055 & 11.745 & 0.078 \\
NGC7619 & 9.790 & 0.026 & 9.723 & 0.014 & 9.877 & 0.023 \\
NGC7653 & 11.198 & 0.053 & 11.292 & 0.043 & 11.510 & 0.100 \\
NGC7691 & 11.155 & 0.071 & 11.230 & 0.055 & 11.330 & 0.119 \\
NGC7771 & 9.811 & 0.018 & 10.005 & 0.013 & 9.954 & 0.022 \\
NGC7803 & 10.976 & 0.048 & 11.544 & 0.038 & 11.305 & 0.050 \\
PGC0035860 & -99.000 & -99.000 & 15.252 & 0.481 & 17.462 & 6.248 \\
PGC0213858 & 14.477 & 0.299 & 14.540 & 0.211 & 14.597 & 0.377 \\
PGC11179 & 11.848 & 0.061 & 12.195 & 0.050 & 12.159 & 0.070 \\
PGC1481751 & 13.159 & 0.145 & 13.859 & 0.199 & 13.132 & 0.191 \\
PGC213672 & 13.431 & 0.192 & 13.638 & 0.135 & 13.910 & 0.272 \\
PGC3086846 & 14.423 & 0.279 & 14.835 & 0.255 & 14.917 & 0.461 \\
PGC34730 & 12.369 & 0.093 & 13.492 & 0.143 & 13.471 & 0.265 \\
PGC37426 & 13.463 & 0.189 & 14.018 & 0.224 & 13.894 & 0.328 \\
SDSSJ004750 & 15.663 & 0.864 & 16.656 & 1.290 & 18.708 & 14.386 \\
SDSSJ025953 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 & -99.000 \\
SDSSJ083516 & -99.000 & -99.000 & 18.462 & 10.831 & -99.000 & -99.000 \\
SDSSJ08535700 & -99.000 & -99.000 & 15.435 & 0.562 & 14.937 & 0.560 \\
SDSSJ120951251947165 & 14.280 & 0.310 & 14.622 & 0.238 & 14.966 & 0.493 \\
SDSSJ161812 & 16.393 & 2.645 & 15.475 & 0.763 & 14.905 & 0.763 \\
SDSSJ170413 & 14.629 & 0.647 & 14.592 & 0.306 & 13.915 & 0.265 \\
UGC00005 & 13.017 & 0.338 & 12.044 & 0.078 & 12.274 & 0.176 \\
UGC00040 & 11.738 & 0.091 & 12.542 & 0.110 & 12.376 & 0.148 \\
UGC00139 & 11.683 & 0.153 & 12.490 & 0.122 & 12.389 & 0.179 \\
UGC00148 & 12.193 & 0.091 & 12.286 & 0.066 & 12.161 & 0.117 \\
UGC01087 & -99.000 & -99.000 & 12.745 & 0.154 & -99.000 & -99.000 \\
UGC02134 & 11.588 & 0.061 & 11.661 & 0.048 & 11.633 & 0.074 \\
UGC02308 & 12.473 & 0.154 & 12.623 & 0.102 & 12.550 & 0.134 \\
UGC02628 & 12.874 & 0.243 & 12.784 & 0.135 & 12.720 & 0.240 \\
UGC02756 & 11.269 & 0.037 & 11.443 & 0.026 & 11.445 & 0.038 \\
UGC02829 & 11.300 & 0.052 & 11.641 & 0.038 & 11.578 & 0.049 \\
UGC02836 & 10.981 & 0.036 & 11.278 & 0.032 & 11.408 & 0.060 \\
UGC03151 & 11.482 & 0.064 & 11.422 & 0.041 & 11.446 & 0.056 \\
UGC03552 & -99.000 & -99.000 & 12.760 & 0.123 & -99.000 & -99.000 \\
UGC03944 & 11.982 & 0.103 & 12.685 & 0.127 & 11.685 & 0.097 \\
UGC04008 & 11.665 & 0.057 & 11.971 & 0.051 & 11.754 & 0.067 \\
UGC04107 & 12.035 & 0.133 & 12.016 & 0.085 & 12.210 & 0.153 \\
UGC04132 & 11.583 & 0.087 & 11.625 & 0.057 & 11.394 & 0.069 \\
UGC04179 & 11.958 & 0.080 & 13.561 & 0.199 & 13.145 & 0.231 \\
UGC04195 & 11.762 & 0.086 & 12.019 & 0.079 & 12.001 & 0.125 \\
UGC04308 & 10.567 & 0.046 & 10.799 & 0.036 & 10.782 & 0.054 \\
UGC04310 & 13.652 & 0.600 & 14.630 & 1.135 & 13.616 & 0.759 \\
UGC04414 & -99.000 & -99.000 & 12.475 & 0.085 & -99.000 & -99.000 \\
UGC04455 & -99.000 & -99.000 & 15.296 & 1.593 & -99.000 & -99.000 \\
UGC04461 & 12.084 & 0.148 & 12.412 & 0.121 & 12.239 & 0.166 \\
UGC04468 & 11.806 & 0.081 & 11.932 & 0.062 & 12.190 & 0.123 \\
UGC05100 & 12.759 & 0.273 & 13.276 & 0.293 & 15.378 & 3.357 \\
UGC05129 & 10.579 & 0.038 & 12.027 & 0.069 & 11.849 & 0.091 \\
UGC05392 & 11.631 & 0.064 & 13.153 & 0.105 & 12.622 & 0.109 \\
UGC05520 & 12.546 & 0.209 & 13.081 & 0.211 & 13.235 & 0.367 \\
UGC05695 & 12.743 & 0.191 & 13.189 & 0.180 & 13.035 & 0.270 \\
UGC06036 & 12.022 & 0.097 & 11.909 & 0.053 & 11.996 & 0.090 \\
UGC06483 & 12.619 & 0.117 & 12.803 & 0.070 & 12.559 & 0.096 \\
UGC06517 & 12.779 & 0.190 & 12.985 & 0.147 & 12.657 & 0.171 \\
UGC06609 & 11.849 & 0.076 & 12.087 & 0.064 & 12.140 & 0.123 \\
UGC07228 & 12.957 & 0.259 & 12.924 & 0.129 & 13.105 & 0.250 \\
UGC08250 & 12.839 & 0.156 & 13.498 & 0.189 & 13.036 & 0.199 \\
UGC08472 & 12.549 & 0.133 & 12.846 & 0.138 & 12.787 & 0.224 \\
UGC08503 & 12.693 & 0.229 & 13.383 & 0.225 & 13.189 & 0.300 \\
UGC08733 & 11.445 & 0.090 & 12.384 & 0.147 & 12.636 & 0.323 \\
UGC08932 & 13.782 & 0.330 & 14.157 & 0.284 & 14.589 & 0.775 \\
UGC09165 & 12.177 & 0.076 & 12.421 & 0.070 & 11.991 & 0.073 \\
UGC09356 & 12.191 & 0.130 & 13.396 & 0.280 & 14.029 & 0.885 \\
UGC09629 & 11.742 & 0.073 & 12.124 & 0.060 & 11.981 & 0.084 \\
UGC09842 & 13.198 & 0.251 & 12.813 & 0.121 & 12.610 & 0.185 \\
UGC10064 & 11.920 & 0.072 & 12.299 & 0.058 & 12.555 & 0.112 \\
UGC10097 & 10.829 & 0.028 & 11.031 & 0.023 & 11.085 & 0.046 \\
UGC10123 & 12.130 & 0.099 & 12.157 & 0.056 & 11.906 & 0.085 \\
UGC10331 & 14.075 & 0.602 & 14.088 & 0.428 & 13.445 & 0.375 \\
UGC10414 & 11.162 & 0.061 & 12.585 & 0.122 & 12.779 & 0.248 \\
UGC1071 & 11.691 & 0.054 & 12.503 & 0.066 & 12.308 & 0.108 \\
UGC11723 & 10.952 & 0.045 & 11.897 & 0.067 & 11.568 & 0.076 \\
UGC12157 & 13.832 & 0.151 & 14.217 & 0.192 & 13.631 & 0.228 \\
UGC12810 & 11.784 & 0.128 & 11.923 & 0.083 & 11.455 & 0.093 \\
UGC12850 & 12.867 & 0.178 & 13.548 & 0.196 & 13.316 & 0.250 \\
UGC2164 & 12.219 & 0.122 & 12.676 & 0.115 & 12.669 & 0.165 \\
UGC6837 & 15.580 & 1.526 & 14.710 & 0.505 & 14.318 & 0.613
\enddata
\end{deluxetable}


==> global_photometry_full.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrr}
\tablecaption{In-house global photometry for SDSS and GALEX.  Only GALEX photometry with SDSS coverage was measured. Given as AB magnitudes; -99 marks negative flux. } \rotate \label{table:global_photometry}
\tablehead{\colhead{Galaxy} & \colhead{$m_u$} & \colhead{$\sigma_{m_u}$} & \colhead{$m_g$} & \colhead{$\sigma_{m_g}$} & \colhead{$m_r$} & \colhead{$\sigma_{m_r}$} & \colhead{$m_i$} & \colhead{$\sigma_{m_i}$} & \colhead{$m_z$} & \colhead{$\sigma_{m_z}$} & \colhead{$m_{NUV}$} & \colhead{$\sigma_{m_{NUV}}$} & \colhead{$m_{FUV}$} & \colhead{$\sigma_{m_{FUV}}$}}
\startdata
2MASSJ00164451 & 19.522 & 0.258 & 17.730 & 0.020 & 16.919 & 0.014 & 16.485 & 0.015 & 16.128 & 0.050 & -99.000 & -99.000 & -99.000 & -99.000 \\
2MASSJ00235669 & 17.894 & 0.054 & 16.737 & 0.005 & 16.492 & 0.007 & 16.280 & 0.009 & 16.109 & 0.028 & 18.676 & 0.048 & 19.239 & 0.106 \\
2MASSJ23243021 & 19.010 & 0.118 & 17.363 & 0.009 & 16.539 & 0.006 & 16.119 & 0.007 & 15.930 & 0.028 & 22.980 & 0.398 & 23.196 & 0.514 \\
2MASXJ00234829 & 16.298 & 0.046 & 15.597 & 0.006 & 15.074 & 0.007 & 14.675 & 0.008 & 14.783 & 0.030 & 17.661 & 0.034 & 18.158 & 0.064 \\
2MASXJ01144386 & 16.983 & 0.071 & 15.902 & 0.008 & 15.286 & 0.007 & 14.940 & 0.008 & 14.734 & 0.034 & 18.174 & 0.056 & 18.523 & 0.092 \\
2MASXJ01403375 & 17.235 & 0.092 & 15.842 & 0.008 & 15.147 & 0.007 & 14.735 & 0.007 & 14.384 & 0.018 & 18.693 & 0.090 & 18.925 & 0.135 \\
2MASXJ02305208 & 17.268 & 0.066 & 16.119 & 0.007 & 15.248 & 0.004 & 14.721 & 0.004 & 14.591 & 0.012 & 19.920 & 0.489 & -99.000 & -99.000 \\
2MASXJ08374557 & 17.472 & 0.077 & 16.399 & 0.011 & 15.936 & 0.011 & 15.509 & 0.011 & 15.342 & 0.033 & 18.813 & 0.097 & 19.552 & 0.212 \\
2MASXJ10525434 & 17.080 & 0.053 & 16.179 & 0.007 & 15.638 & 0.007 & 15.341 & 0.008 & 15.151 & 0.034 & -99.000 & -99.000 & -99.000 & -99.000 \\
2MASXJ11123493 & 17.033 & 0.052 & 16.064 & 0.007 & 15.447 & 0.006 & 15.068 & 0.007 & 14.688 & 0.025 & 18.422 & 0.050 & 19.284 & 0.163 \\
2MASXJ11500404 & 17.178 & 0.039 & 15.635 & 0.005 & 14.875 & 0.003 & 14.513 & 0.004 & 14.262 & 0.009 & 20.588 & 0.222 & -99.000 & -99.000 \\
2MASXJ12095669 & 17.249 & 0.048 & 15.797 & 0.005 & 14.970 & 0.004 & 14.565 & 0.004 & 14.281 & 0.012 & -99.000 & -99.000 & -99.000 & -99.000 \\
2MASXJ12385810 & 17.352 & 0.079 & 16.419 & 0.011 & 15.782 & 0.010 & 15.459 & 0.011 & 15.080 & 0.028 & 19.298 & 0.116 & 19.734 & 0.248 \\
2MASXJ15024995 & 17.948 & 0.092 & 16.413 & 0.012 & 15.845 & 0.009 & 15.433 & 0.010 & 15.326 & 0.030 & -99.000 & -99.000 & -99.000 & -99.000 \\
2MASXJ15393305 & 16.579 & 0.054 & 15.286 & 0.005 & 14.449 & 0.004 & 14.054 & 0.004 & 13.822 & 0.011 & 18.930 & 0.101 & 22.090 & 1.304 \\
2MASXJ15570268 & 17.752 & 0.083 & 16.374 & 0.008 & 15.580 & 0.006 & 15.280 & 0.007 & 14.869 & 0.025 & 20.112 & 0.295 & 20.519 & 0.546 \\
2MASXJ16065563 & 16.311 & 0.056 & 15.230 & 0.008 & 14.891 & 0.008 & 14.522 & 0.008 & 14.502 & 0.036 & 17.177 & 0.037 & 17.599 & 0.107 \\
2MASXJ16152860 & 18.085 & 0.134 & 16.823 & 0.012 & 16.104 & 0.010 & 15.700 & 0.012 & 15.442 & 0.032 & 20.148 & 0.189 & 21.911 & 1.727 \\
2MASXJ16301506 & 16.960 & 0.064 & 15.789 & 0.008 & 15.144 & 0.006 & 14.761 & 0.006 & 14.468 & 0.022 & 18.730 & 0.105 & 19.668 & 0.294 \\
2MASXJ17100856 & 17.798 & 0.076 & 16.191 & 0.006 & 15.471 & 0.005 & 15.108 & 0.005 & 14.809 & 0.019 & 21.724 & 0.668 & 20.789 & 0.429 \\
2MASXJ21352164 & 17.328 & 0.130 & 15.943 & 0.009 & 15.062 & 0.006 & 14.499 & 0.005 & 14.250 & 0.015 & -99.000 & -99.000 & 20.613 & 1.575 \\
2MASXJ22532475 & 17.066 & 0.077 & 15.499 & 0.005 & 14.814 & 0.005 & 14.483 & 0.005 & 14.212 & 0.020 & 18.084 & 0.059 & 19.099 & 0.163 \\
2MASXJ23024668 & 17.992 & 0.104 & 16.219 & 0.006 & 15.345 & 0.004 & 14.902 & 0.004 & 14.561 & 0.010 & 21.219 & 0.097 & 22.513 & 0.326 \\
ARP143 & 13.572 & 0.007 & 12.328 & 0.001 & 11.720 & 0.001 & 11.417 & 0.001 & 11.179 & 0.004 & 14.712 & 0.010 & 15.149 & 0.019 \\
ARP70 & 15.566 & 0.047 & 14.259 & 0.004 & 13.531 & 0.003 & 13.068 & 0.003 & 12.797 & 0.010 & 17.264 & 0.033 & 18.020 & 0.075
\enddata
\end{deluxetable}


==> local_photometry.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrr}
\tablecaption{In-house local 1 kpc photometry for SDSS and GALEX.  Only GALEX photometry with SDSS coverage were measured. Given as AB magnitudes; -99 marks negative flux. The first 25 entries are shown here. A full version of this table is available online.} \rotate \label{table:local_photometry}
\tablehead{\colhead{SN} & \colhead{$m_u$} & \colhead{$\sigma_{m_u}$} & \colhead{$m_g$} & \colhead{$\sigma_{m_g}$} & \colhead{$m_r$} & \colhead{$\sigma_{m_r}$} & \colhead{$m_i$} & \colhead{$\sigma_{m_i}$} & \colhead{$m_z$} & \colhead{$\sigma_{m_z}$} & \colhead{$m_{NUV}$} & \colhead{$\sigma_{m_{NUV}}$} & \colhead{$m_{FUV}$} & \colhead{$\sigma_{m_{FUV}}$}}
\startdata
ASASSN-13dd & 17.600 & 0.013 & 15.808 & 0.002 & 15.062 & 0.001 & 14.674 & 0.001 & 14.391 & 0.003 & 20.548 & 0.039 & 22.390 & 0.167 \\
ASASSN-14ay & 21.904 & 0.243 & 20.128 & 0.018 & 19.400 & 0.014 & 19.043 & 0.016 & 18.769 & 0.059 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-14fj & 19.409 & 0.060 & 18.788 & 0.012 & 18.508 & 0.014 & 18.358 & 0.017 & 18.400 & 0.064 & 20.126 & 0.115 & 20.531 & 0.241 \\
ASASSN-14kd & 19.224 & 0.039 & 17.862 & 0.005 & 17.237 & 0.004 & 16.908 & 0.004 & 16.631 & 0.013 & 21.214 & 0.171 & 21.883 & 0.399 \\
ASASSN-15cb & 19.706 & 0.030 & 18.556 & 0.007 & 18.000 & 0.005 & 17.718 & 0.006 & 17.462 & 0.014 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15cd & 19.075 & 0.021 & 18.116 & 0.005 & 17.917 & 0.005 & 17.767 & 0.006 & 17.660 & 0.015 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15db & 15.270 & 0.004 & 14.769 & 0.001 & 14.410 & 0.001 & 14.351 & 0.001 & 14.192 & 0.003 & 16.265 & 0.011 & 16.756 & 0.032 \\
ASASSN-15dd & 19.418 & 0.045 & 17.597 & 0.005 & 16.833 & 0.003 & 16.434 & 0.003 & 16.109 & 0.007 & 22.960 & 0.314 & 23.371 & 0.834 \\
ASASSN-15fj & 19.261 & 0.031 & 17.417 & 0.004 & 16.693 & 0.003 & 16.320 & 0.003 & 16.054 & 0.007 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15ga & 15.463 & 0.004 & 13.552 & 0.001 & 12.699 & 0.000 & 12.270 & 0.000 & 11.930 & 0.001 & 18.812 & 0.041 & 20.119 & 0.211 \\
ASASSN-15tz & 22.743 & 1.033 & 20.996 & 0.068 & 20.181 & 0.047 & 19.815 & 0.044 & 19.524 & 0.120 & 21.628 & 0.505 & -99.000 & -99.000 \\
ASASSN14-iu & 17.628 & 0.010 & 15.752 & 0.002 & 14.907 & 0.001 & 14.497 & 0.001 & 14.203 & 0.002 & 21.720 & 0.184 & 22.900 & 0.800 \\
ASASSN14lo & 21.550 & 0.304 & 20.177 & 0.030 & 19.791 & 0.031 & 19.546 & 0.040 & 19.893 & 0.198 & 22.465 & 0.195 & 26.354 & 6.883 \\
CSP13N & 23.322 & 0.563 & 23.186 & 0.179 & 22.642 & 0.164 & 22.235 & 0.160 & 22.619 & 0.821 & 24.751 & 1.127 & -99.000 & -99.000 \\
CSS140501-J170414+174839 & 27.307 & 13.170 & nan & -1.549 & nan & -1.882 & 26.448 & 5.735 & nan & -0.615 & 26.078 & 2.696 & -99.000 & -99.000 \\
LSQ12fhh & 19.823 & 0.062 & 18.337 & 0.007 & 17.505 & 0.005 & 17.103 & 0.004 & 16.746 & 0.011 & 21.965 & 0.068 & 22.877 & 0.257 \\
LSQ12gef & 23.193 & 0.566 & 21.272 & 0.037 & 20.626 & 0.029 & 20.168 & 0.028 & 19.929 & 0.079 & 24.510 & 0.854 & 23.876 & 1.012 \\
LSQ13vy & 22.303 & 0.337 & 21.553 & 0.064 & 21.222 & 0.063 & 20.858 & 0.065 & 20.363 & 0.189 & 23.081 & 0.389 & 23.409 & 1.180 \\
LSQ14Q & 23.460 & 0.506 & 22.599 & 0.085 & 22.378 & 0.106 & 22.085 & 0.132 & 22.659 & 0.928 & 24.952 & 1.284 & 25.520 & 2.769 \\
LSQ14ajn & 19.672 & 0.053 & 18.022 & 0.006 & 17.285 & 0.004 & 16.929 & 0.004 & 16.628 & 0.009 & 22.508 & 0.386 & 23.734 & 1.161 \\
LSQ14azy & 22.386 & 0.289 & 20.771 & 0.025 & 20.251 & 0.024 & 19.912 & 0.027 & 19.639 & 0.095 & 22.975 & 0.316 & 24.471 & 1.553 \\
LSQ15aae & 24.486 & 2.068 & 23.294 & 0.240 & 22.585 & 0.177 & 22.094 & 0.168 & 21.256 & 0.360 & -99.000 & -99.000 & -99.000 & -99.000 \\
LSQ15agh & 23.337 & 0.498 & 22.509 & 0.075 & 22.310 & 0.094 & 22.015 & 0.114 & 22.097 & 0.584 & -99.000 & -99.000 & -99.000 & -99.000 \\
PS15aot & 20.891 & 0.107 & 18.844 & 0.008 & 17.988 & 0.006 & 17.578 & 0.006 & 17.244 & 0.017 & 23.818 & 0.188 & 24.184 & 0.376 \\
PS15dov & 17.268 & 0.018 & 16.106 & 0.003 & 15.557 & 0.002 & 15.318 & 0.002 & 15.092 & 0.005 & 18.247 & 0.152 & 19.275 & 0.250
\enddata
\end{deluxetable}


==> local_photometry_full.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrr}
\tablecaption{In-house local 1 kpc photometry for SDSS and GALEX.  Only GALEX photometry with SDSS coverage were measured. Given as AB magnitudes; -99 marks negative flux. } \rotate \label{table:local_photometry}
\tablehead{\colhead{SN} & \colhead{$m_u$} & \colhead{$\sigma_{m_u}$} & \colhead{$m_g$} & \colhead{$\sigma_{m_g}$} & \colhead{$m_r$} & \colhead{$\sigma_{m_r}$} & \colhead{$m_i$} & \colhead{$\sigma_{m_i}$} & \colhead{$m_z$} & \colhead{$\sigma_{m_z}$} & \colhead{$m_{NUV}$} & \colhead{$\sigma_{m_{NUV}}$} & \colhead{$m_{FUV}$} & \colhead{$\sigma_{m_{FUV}}$}}
\startdata
ASASSN-13dd & 17.600 & 0.013 & 15.808 & 0.002 & 15.062 & 0.001 & 14.674 & 0.001 & 14.391 & 0.003 & 20.548 & 0.039 & 22.390 & 0.167 \\
ASASSN-14ay & 21.904 & 0.243 & 20.128 & 0.018 & 19.400 & 0.014 & 19.043 & 0.016 & 18.769 & 0.059 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-14fj & 19.409 & 0.060 & 18.788 & 0.012 & 18.508 & 0.014 & 18.358 & 0.017 & 18.400 & 0.064 & 20.126 & 0.115 & 20.531 & 0.241 \\
ASASSN-14kd & 19.224 & 0.039 & 17.862 & 0.005 & 17.237 & 0.004 & 16.908 & 0.004 & 16.631 & 0.013 & 21.214 & 0.171 & 21.883 & 0.399 \\
ASASSN-15cb & 19.706 & 0.030 & 18.556 & 0.007 & 18.000 & 0.005 & 17.718 & 0.006 & 17.462 & 0.014 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15cd & 19.075 & 0.021 & 18.116 & 0.005 & 17.917 & 0.005 & 17.767 & 0.006 & 17.660 & 0.015 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15db & 15.270 & 0.004 & 14.769 & 0.001 & 14.410 & 0.001 & 14.351 & 0.001 & 14.192 & 0.003 & 16.265 & 0.011 & 16.756 & 0.032 \\
ASASSN-15dd & 19.418 & 0.045 & 17.597 & 0.005 & 16.833 & 0.003 & 16.434 & 0.003 & 16.109 & 0.007 & 22.960 & 0.314 & 23.371 & 0.834 \\
ASASSN-15fj & 19.261 & 0.031 & 17.417 & 0.004 & 16.693 & 0.003 & 16.320 & 0.003 & 16.054 & 0.007 & -99.000 & -99.000 & -99.000 & -99.000 \\
ASASSN-15ga & 15.463 & 0.004 & 13.552 & 0.001 & 12.699 & 0.000 & 12.270 & 0.000 & 11.930 & 0.001 & 18.812 & 0.041 & 20.119 & 0.211 \\
ASASSN-15tz & 22.743 & 1.033 & 20.996 & 0.068 & 20.181 & 0.047 & 19.815 & 0.044 & 19.524 & 0.120 & 21.628 & 0.505 & -99.000 & -99.000 \\
ASASSN14-iu & 17.628 & 0.010 & 15.752 & 0.002 & 14.907 & 0.001 & 14.497 & 0.001 & 14.203 & 0.002 & 21.720 & 0.184 & 22.900 & 0.800 \\
ASASSN14lo & 21.550 & 0.304 & 20.177 & 0.030 & 19.791 & 0.031 & 19.546 & 0.040 & 19.893 & 0.198 & 22.465 & 0.195 & 26.354 & 6.883 \\
CSP13N & 23.322 & 0.563 & 23.186 & 0.179 & 22.642 & 0.164 & 22.235 & 0.160 & 22.619 & 0.821 & 24.751 & 1.127 & -99.000 & -99.000 \\
CSS140501-J170414+174839 & 27.307 & 13.170 & nan & -1.549 & nan & -1.882 & 26.448 & 5.735 & nan & -0.615 & 26.078 & 2.696 & -99.000 & -99.000 \\
LSQ12fhh & 19.823 & 0.062 & 18.337 & 0.007 & 17.505 & 0.005 & 17.103 & 0.004 & 16.746 & 0.011 & 21.965 & 0.068 & 22.877 & 0.257 \\
LSQ12gef & 23.193 & 0.566 & 21.272 & 0.037 & 20.626 & 0.029 & 20.168 & 0.028 & 19.929 & 0.079 & 24.510 & 0.854 & 23.876 & 1.012 \\
LSQ13vy & 22.303 & 0.337 & 21.553 & 0.064 & 21.222 & 0.063 & 20.858 & 0.065 & 20.363 & 0.189 & 23.081 & 0.389 & 23.409 & 1.180 \\
LSQ14Q & 23.460 & 0.506 & 22.599 & 0.085 & 22.378 & 0.106 & 22.085 & 0.132 & 22.659 & 0.928 & 24.952 & 1.284 & 25.520 & 2.769 \\
LSQ14ajn & 19.672 & 0.053 & 18.022 & 0.006 & 17.285 & 0.004 & 16.929 & 0.004 & 16.628 & 0.009 & 22.508 & 0.386 & 23.734 & 1.161 \\
LSQ14azy & 22.386 & 0.289 & 20.771 & 0.025 & 20.251 & 0.024 & 19.912 & 0.027 & 19.639 & 0.095 & 22.975 & 0.316 & 24.471 & 1.553 \\
LSQ15aae & 24.486 & 2.068 & 23.294 & 0.240 & 22.585 & 0.177 & 22.094 & 0.168 & 21.256 & 0.360 & -99.000 & -99.000 & -99.000 & -99.000 \\
LSQ15agh & 23.337 & 0.498 & 22.509 & 0.075 & 22.310 & 0.094 & 22.015 & 0.114 & 22.097 & 0.584 & -99.000 & -99.000 & -99.000 & -99.000 \\
PS15aot & 20.891 & 0.107 & 18.844 & 0.008 & 17.988 & 0.006 & 17.578 & 0.006 & 17.244 & 0.017 & 23.818 & 0.188 & 24.184 & 0.376 \\
PS15dov & 17.268 & 0.018 & 16.106 & 0.003 & 15.557 & 0.002 & 15.318 & 0.002 & 15.092 & 0.005 & 18.247 & 0.152 & 19.275 & 0.250
\enddata
\end{deluxetable}


==> local_sfr_mass.tex <==
\begin{deluxetable}{lrrrr}
\tablecaption{Local 1 kpc aperture SFR ($M_{\odot} \text{yr}^{-1}$) and stellar mass estimates ($\log_{10}(M/M_{\odot})$).Mass estimates are from FAST++ using SDSS and GALEX photometry. Only SNe with SDSS and GALEX coverage were included.The first 25 entries are shown here. A full version of this table is available online.} \rotate \label{table:local_sfr_mass}
\tablehead{\colhead{SN} & \colhead{H$\alpha$ SFR} & \colhead{NUV SFR} & \colhead{FUV SFR} & \colhead{FAST++ Mass}}
\startdata
ASASSN-13dd & 0.000 & 0.009 & 0.002 & 9.500 \\
ASASSN-14ay & 0.000 & -0.289 & -0.284 & 8.340 \\
ASASSN-14fj & 0.008 & 0.013 & 0.009 & 7.100 \\
ASASSN-14kd & 0.018 & 0.018 & 0.010 & 9.050 \\
ASASSN-15cb & 0.052 & -0.533 & -0.519 & 9.100 \\
ASASSN-15cd & 0.025 & -0.382 & -0.373 & 8.470 \\
ASASSN-15db & 0.108 & 0.347 & 0.221 & 8.330 \\
ASASSN-15dd & 0.000 & 0.004 & 0.002 & 9.250 \\
ASASSN-15fj & 0.001 & -0.618 & -0.600 & 9.650 \\
ASASSN-15ga & 0.007 & 0.012 & 0.004 & 9.800 \\
ASASSN-15tz & 0.001 & 0.011 & -0.385 & 8.050 \\
LSQ12fhh & 0.008 & 0.008 & 0.003 & 9.250 \\
LSQ12gef & 0.010 & 0.006 & 0.012 & 8.530 \\
LSQ13vy & 0.002 & 0.010 & 0.007 & 7.250 \\
LSQ14azy & 0.001 & 0.013 & 0.003 & 8.180 \\
LSQ14q & 0.005 & 0.005 & 0.003 & 7.120 \\
LSQ15aae & 0.005 & -1.204 & -1.134 & 7.340 \\
LSQ15agh & 0.000 & -1.174 & -1.151 & 7.080 \\
PS15aot & 0.000 & 0.003 & 0.002 & 9.030 \\
PS15dov & 0.121 & 0.130 & 0.050 & 9.200 \\
PTF09cjq & 0.020 & 0.020 & 0.014 & 8.970 \\
PTF10hcw & 0.002 & 0.009 & 0.004 & 8.840 \\
PTF11kju & 0.139 & 0.057 & 0.015 & 9.560 \\
PTF11phk & 0.031 & 0.038 & 0.037 & 8.500 \\
PTF11ppn & 0.000 & -3.759 & -3.319 & 8.980
\enddata
\end{deluxetable}


==> local_sfr_mass_full.tex <==
\begin{deluxetable}{lrrrr}
\tablecaption{Local 1 kpc aperture SFR ($M_{\odot} \text{yr}^{-1}$) and stellar mass estimates ($\log_{10}(M/M_{\odot})$).Mass estimates are from FAST++ using SDSS and GALEX photometry. Only SNe with SDSS and GALEX coverage were included.} \rotate \label{table:local_sfr_mass}
\tablehead{\colhead{SN} & \colhead{H$\alpha$ SFR} & \colhead{NUV SFR} & \colhead{FUV SFR} & \colhead{FAST++ Mass}}
\startdata
ASASSN-13dd & 0.000 & 0.009 & 0.002 & 9.500 \\
ASASSN-14ay & 0.000 & -0.289 & -0.284 & 8.340 \\
ASASSN-14fj & 0.008 & 0.013 & 0.009 & 7.100 \\
ASASSN-14kd & 0.018 & 0.018 & 0.010 & 9.050 \\
ASASSN-15cb & 0.052 & -0.533 & -0.519 & 9.100 \\
ASASSN-15cd & 0.025 & -0.382 & -0.373 & 8.470 \\
ASASSN-15db & 0.108 & 0.347 & 0.221 & 8.330 \\
ASASSN-15dd & 0.000 & 0.004 & 0.002 & 9.250 \\
ASASSN-15fj & 0.001 & -0.618 & -0.600 & 9.650 \\
ASASSN-15ga & 0.007 & 0.012 & 0.004 & 9.800 \\
ASASSN-15tz & 0.001 & 0.011 & -0.385 & 8.050 \\
LSQ12fhh & 0.008 & 0.008 & 0.003 & 9.250 \\
LSQ12gef & 0.010 & 0.006 & 0.012 & 8.530 \\
LSQ13vy & 0.002 & 0.010 & 0.007 & 7.250 \\
LSQ14azy & 0.001 & 0.013 & 0.003 & 8.180 \\
LSQ14q & 0.005 & 0.005 & 0.003 & 7.120 \\
LSQ15aae & 0.005 & -1.204 & -1.134 & 7.340 \\
LSQ15agh & 0.000 & -1.174 & -1.151 & 7.080 \\
PS15aot & 0.000 & 0.003 & 0.002 & 9.030 \\
PS15dov & 0.121 & 0.130 & 0.050 & 9.200 \\
PTF09cjq & 0.020 & 0.020 & 0.014 & 8.970 \\
PTF10hcw & 0.002 & 0.009 & 0.004 & 8.840 \\
PTF11kju & 0.139 & 0.057 & 0.015 & 9.560 \\
PTF11phk & 0.031 & 0.038 & 0.037 & 8.500 \\
PTF11ppn & 0.000 & -3.759 & -3.319 & 8.980 \\
PTF12ikt & 0.004 & 0.008 & 0.009 & 6.940 \\
SN1954b & 0.041 & 0.031 & 0.020 & 8.090 \\
SN1960m & 0.003 & 0.013 & 0.009 & 7.930 \\
SN1963j & 0.002 & -0.003 & -0.003 & 8.720 \\
SN1969c & 0.004 & 0.014 & 0.007 & 8.750 \\
SN1970j & 0.000 & 0.001 & -0.067 & 8.830 \\
SN1971k & 0.019 & 0.005 & 0.006 & 6.830 \\
SN1971p & 0.000 & 0.002 & 0.001 & 8.600 \\
SN1981g & 0.000 & -0.156 & -0.155 & 8.670 \\
SN1984l & 0.007 & 0.023 & 0.020 & 7.690 \\
SN1986n & 0.011 & 0.054 & 0.036 & 8.400 \\
SN1988l & 0.020 & -0.011 & -0.011 & 8.490 \\
SN1989a & 0.001 & 0.005 & 0.003 & 8.020 \\
SN1991ak & 0.002 & 0.003 & 0.002 & 8.050 \\
SN1991n & 0.257 & 0.719 & 0.535 & 8.950 \\
SN1992bf & 0.001 & 0.005 & 0.001 & 8.930 \\
SN1992i & 0.002 & 0.001 & 0.001 & 6.640 \\
SN1993ae & 0.000 & -0.130 & -0.126 & 7.570 \\
SN1993n & 0.006 & 0.016 & 0.010 & 7.770 \\
SN1994n & 0.002 & 0.011 & 0.008 & 8.050 \\
SN1995l & 0.000 & 0.002 & 0.001 & 8.320 \\
SN1997cw & 0.005 & 0.032 & 0.015 & 8.870 \\
SN1997cx & 0.007 & 0.023 & 0.018 & 7.890 \\
SN1997dn & 0.007 & -0.005 & -0.005 & -- \\
SN1997ef & 0.018 & -0.047 & -0.045 & 7.530 \\
SN1998aq & 0.000 & -0.004 & -0.004 & 8.790 \\
SN1998ar & 0.001 & 0.013 & 0.009 & 7.630 \\
SN1999aa & 0.003 & 0.009 & 0.006 & 8.150 \\
SN1999ac & 0.006 & 0.004 & 0.003 & 7.260 \\
SN1999bg & 0.004 & 0.009 & 0.006 & 6.960 \\
SN1999di & 0.008 & 0.027 & 0.018 & 8.410 \\
SN1999dk & 0.003 & -0.081 & -0.078 & 7.460 \\
SN1999dq & 0.091 & 0.065 & 0.029 & 9.370 \\
SN1999ej & 0.000 & 0.000 & -0.075 & 8.210 \\
SN1999gd & 0.001 & 0.006 & 0.003 & 7.940 \\
SN1999ge & 0.006 & 0.017 & 0.006 & 8.460 \\
SN2000ce & 0.003 & 0.005 & 0.003 & 8.080 \\
SN2000da & 0.018 & 0.012 & 0.010 & 8.790 \\
SN2000de & 0.069 & 0.100 & 0.075 & 8.800 \\
SN2000ey & 0.039 & 0.064 & 0.047 & 9.720 \\
SN2000fn & 0.007 & -0.071 & -0.070 & 8.380 \\
SN2000ft & 1.130 & 1.897 & 1.733 & 9.110 \\
SN2000l & 0.005 & -0.040 & -0.039 & 7.610 \\
SN2001ch & 0.014 & 0.040 & 0.025 & 7.300 \\
SN2001co & 0.009 & 0.005 & 0.004 & 8.480 \\
SN2001en & 0.001 & 0.007 & 0.002 & 8.620 \\
SN2001fe & 0.002 & 0.013 & 0.008 & 8.640 \\
SN2001h & 0.006 & -0.116 & -0.111 & -- \\
SN2001i & 0.171 & 0.105 & 0.041 & 9.270 \\
SN2001ic & 0.000 & 0.004 & -0.801 & 8.350 \\
SN2002au & 0.014 & 0.014 & 0.008 & 8.360 \\
SN2002ce & 0.015 & -0.016 & -0.016 & 7.270 \\
SN2002ee & 0.002 & 0.003 & 0.002 & 7.610 \\
SN2002ha & 0.000 & 0.002 & 0.001 & 8.050 \\
SN2002ho & 0.004 & 0.017 & -0.023 & 8.570 \\
SN2002jg & 0.003 & 0.020 & 0.018 & 8.070 \\
SN2002ji & 0.012 & 0.032 & 0.020 & 8.480 \\
SN2003bp & 0.007 & 0.021 & 0.011 & 8.330 \\
SN2003dr & 0.001 & 0.002 & 0.002 & 7.290 \\
SN2003ds & 0.133 & -0.252 & -0.249 & 8.460 \\
SN2003dt & 0.005 & 0.003 & 0.001 & 8.180 \\
SN2003el & 0.009 & 0.007 & 0.004 & 8.480 \\
SN2003g & 0.003 & 0.009 & 0.005 & 8.200 \\
SN2003hg & 0.055 & 0.019 & 0.008 & 9.430 \\
SN2003i & 0.009 & -0.112 & -0.108 & 8.100 \\
SN2003ih & 0.057 & 0.016 & 0.005 & 8.770 \\
SN2003it & 0.001 & 0.006 & 0.003 & 8.060 \\
SN2003lc & 0.000 & 0.010 & 0.001 & 10.370 \\
SN2003ld & 0.044 & -0.078 & -0.074 & 8.850 \\
SN2003lq & 0.004 & -0.201 & 0.002 & 7.300 \\
SN2004bs & 0.030 & 0.080 & 0.039 & 8.700 \\
SN2004ci & 0.016 & 0.027 & 0.015 & 8.930 \\
SN2004di & 0.000 & -0.114 & -0.113 & 8.060 \\
SN2004fd & 0.000 & 0.014 & 0.004 & 9.790 \\
SN2004g & 0.000 & 0.010 & 0.006 & 7.400 \\
SN2004gj & 0.004 & 0.016 & 0.006 & 7.860 \\
SN2004gu & 0.002 & 0.002 & 0.001 & 8.510 \\
SN2005au & 0.016 & 0.035 & 0.036 & 8.040 \\
SN2005az & 0.029 & 0.050 & 0.037 & 8.720 \\
SN2005ci & 0.014 & 0.022 & 0.014 & 8.550 \\
SN2005db & 0.040 & 0.034 & 0.017 & 8.760 \\
SN2005dp & 0.003 & 0.023 & 0.016 & 7.760 \\
SN2005en & 0.036 & 0.034 & 0.025 & 8.240 \\
SN2005eo & 0.029 & 0.015 & 0.007 & 8.420 \\
SN2005eq & 0.000 & 0.002 & 0.001 & 7.640 \\
SN2005ip & 0.030 & 0.024 & 0.015 & 8.420 \\
SN2005kc & 0.017 & 0.021 & 0.011 & 8.960 \\
SN2005kk & 0.005 & 0.026 & 0.018 & 7.410 \\
SN2005lt & 0.009 & 0.011 & 0.008 & 7.090 \\
SN2005ly & 0.005 & 0.004 & 0.005 & 7.800 \\
SN2005mc & 0.001 & 0.003 & 0.001 & 8.880 \\
SN2005w & 0.001 & 0.004 & 0.002 & -- \\
SN2006am & 0.027 & 0.037 & 0.019 & 8.260 \\
SN2006bd & 0.000 & 0.001 & 0.000 & 8.230 \\
SN2006be & 0.005 & 0.013 & 0.011 & 8.120 \\
SN2006cm & 0.011 & 0.006 & 0.003 & 9.420 \\
SN2006ct & 0.001 & -0.294 & -0.290 & 8.710 \\
SN2006dy & 0.001 & 0.004 & 0.003 & 8.560 \\
SN2006ee & 0.001 & 0.002 & 0.001 & 8.650 \\
SN2006eh & 0.008 & 0.024 & -0.565 & 8.880 \\
SN2006jd & 0.003 & -0.132 & -0.126 & 7.090 \\
SN2006kf & 0.000 & 0.001 & -0.564 & 7.930 \\
SN2006lc & 0.008 & 0.014 & 0.007 & 8.740 \\
SN2006lv & 0.007 & 0.016 & 0.013 & 8.360 \\
SN2006n & 0.001 & 0.004 & 0.000 & 9.360 \\
SN2006qp & 0.002 & 0.008 & 0.007 & 7.350 \\
SN2006te & 0.000 & 0.018 & 0.008 & 8.260 \\
SN2007a & 0.022 & 0.031 & 0.018 & 8.800 \\
SN2007ag & 0.008 & -0.135 & -0.132 & 8.560 \\
SN2007ay & 0.003 & 0.006 & 0.006 & 7.380 \\
SN2007bd & 0.003 & 0.013 & 0.001 & 8.580 \\
SN2007bz & 0.018 & 0.054 & 0.036 & 8.070 \\
SN2007cm & 0.001 & -0.080 & -0.079 & 7.860 \\
SN2007hj & 0.001 & -0.095 & -0.089 & 8.690 \\
SN2007hu & 0.000 & 0.001 & -0.438 & 9.270 \\
SN2007jd & 0.002 & 0.007 & -2.384 & 7.790 \\
SN2007kj & 0.005 & 0.011 & 0.007 & 8.800 \\
SN2007n & 0.001 & 0.005 & 0.003 & 8.520 \\
SN2007q & 0.003 & 0.008 & 0.002 & 8.860 \\
SN2007r & 0.000 & 0.022 & 0.011 & 9.310 \\
SN2007rz & 0.102 & -0.183 & 0.053 & 8.990 \\
SN2007sa & 0.000 & -0.007 & -0.007 & 9.160 \\
SN2007ux & 0.000 & 0.002 & -0.320 & 8.280 \\
SN2008b & 0.003 & 0.010 & 0.013 & 7.510 \\
SN2008bi & 0.002 & 0.007 & 0.006 & 9.560 \\
SN2008bz & 0.001 & -1.189 & 0.000 & 6.700 \\
SN2008dr & 0.001 & 0.003 & 0.001 & 8.470 \\
SN2008dt & 0.000 & 0.003 & -0.438 & 8.980 \\
SN2008dw & 0.006 & 0.048 & -0.043 & 7.650 \\
SN2008ec & 0.006 & 0.018 & 0.007 & 8.430 \\
SN2008gj & 0.006 & 0.007 & 0.002 & 7.640 \\
SN2008hv & 0.000 & 0.000 & 0.000 & 8.240 \\
SN2008ie & 0.002 & 0.007 & 0.004 & 8.580 \\
SN2008l & 0.000 & 0.000 & -0.266 & 8.490 \\
SN2009az & 0.000 & 0.002 & 0.001 & 8.940 \\
SN2009cz & 0.000 & 0.004 & 0.001 & 8.110 \\
SN2009dc & 0.000 & -0.197 & -0.186 & 6.830 \\
SN2009fk & 0.021 & 0.036 & 0.016 & 9.210 \\
SN2009fl & 0.000 & -0.237 & -0.235 & 8.570 \\
SN2009ie & 0.001 & 0.003 & 0.002 & 7.120 \\
SN2009iq & 0.007 & 0.004 & -0.564 & 8.430 \\
SN2009lf & 0.000 & -0.404 & -0.387 & 7.740 \\
SN2009p & 0.018 & -0.230 & -0.221 & 8.840 \\
SN2010fv & 0.001 & 0.012 & 0.002 & 8.600 \\
SN2010iz & 0.010 & 0.026 & 0.012 & 8.220 \\
SN2011aq & 0.290 & -0.020 & -0.017 & 9.660 \\
SN2011bm & 0.009 & 0.039 & 0.036 & 7.630 \\
SN2011cj & 0.012 & 0.048 & 0.038 & 7.880 \\
SN2011ck & 0.010 & -0.014 & 0.013 & 8.050 \\
SN2011cl & 0.000 & 0.003 & -0.200 & 5.600 \\
SN2011gd & 0.214 & -0.034 & -0.032 & 9.670 \\
SN2011hr & 0.037 & 0.036 & 0.022 & 9.210 \\
SN2011im & 0.001 & 0.002 & 0.001 & 7.770 \\
SN2011jf & 0.037 & 0.002 & -0.179 & 8.140 \\
SN2011jg & 0.007 & 0.019 & 0.016 & 7.980 \\
SN2012an & 0.003 & 0.004 & 0.004 & 6.970 \\
SN2012as & 0.004 & 0.006 & 0.004 & 7.730 \\
SN2012bh & 0.000 & 0.001 & 0.000 & 6.800 \\
SN2012bp & 0.001 & 0.002 & 0.004 & 6.520 \\
SN2012c & 0.027 & 0.033 & 0.017 & 8.730 \\
SN2012cd & 0.002 & -0.043 & -0.042 & 6.300 \\
SN2012ei & 0.000 & -0.012 & 0.000 & 8.600 \\
SN2012et & 0.018 & 0.027 & 0.021 & 8.510 \\
SN2012fb & 0.004 & 0.005 & 0.000 & 7.640 \\
SN2012fk & 0.004 & 0.000 & -0.738 & 7.740 \\
SN2012go & 0.006 & -0.478 & -0.451 & 8.620 \\
SN2012hl & 0.002 & -0.444 & -0.422 & 7.920 \\
SN2012t & 0.058 & 0.024 & 0.016 & 8.990 \\
SN2013ac & 0.018 & -0.247 & 0.004 & 7.130 \\
SN2013aj & 0.002 & 0.010 & 0.006 & 8.840 \\
SN2013ar & 0.017 & 0.005 & -0.903 & 7.240 \\
SN2013ce & 0.008 & 0.018 & 0.009 & 6.660 \\
SN2013cf & 0.002 & -0.107 & 0.002 & 8.350 \\
SN2013di & 0.003 & 0.008 & 0.003 & 8.150 \\
SN2013gl & 0.065 & 0.081 & 0.062 & 8.880 \\
SN2013gq & 0.001 & 0.007 & 0.002 & 9.340 \\
SN2013gv & 0.000 & 0.000 & -0.882 & 7.880 \\
SN2013he & 0.041 & -0.222 & -0.219 & 8.500 \\
SN2013hh & 0.001 & -0.053 & -0.052 & 7.940 \\
SN2013n & 0.000 & 0.004 & 0.001 & 9.390 \\
SN2013t & 0.001 & 0.004 & 0.002 & 7.330 \\
SN2013u & 0.039 & 0.046 & 0.020 & 8.550 \\
SN2014aa & 0.015 & 0.006 & 0.002 & 9.370 \\
SN2014ac & 0.006 & 0.013 & -0.269 & 8.530 \\
SN2014as & 0.011 & 0.021 & -0.043 & 7.050 \\
SN2014az & 0.003 & 0.009 & 0.007 & 7.880 \\
SN2014cv & 0.028 & 0.005 & -0.044 & 9.600 \\
SN2014ee & 0.021 & 0.012 & 0.006 & 8.260 \\
SN2014ek & 0.023 & -0.214 & -0.204 & 8.950 \\
SN2014ev & 0.004 & 0.007 & 0.015 & 7.920 \\
SN2015ab & 0.000 & 0.002 & 0.001 & 8.960 \\
SN2015bb & 0.005 & 0.009 & 0.009 & 8.710 \\
SN2015bf & 0.007 & -0.083 & 0.015 & 9.900 \\
SN2015z & 0.009 & 0.016 & 0.013 & 7.800 \\
SN2016aqw & 0.002 & 0.003 & 0.001 & 8.730 \\
SN2016bam & 0.033 & 0.017 & 0.007 & 7.870 \\
SN2016cvw & 0.000 & -0.701 & -0.658 & 8.460 \\
SN2016eob & 0.004 & 0.007 & 0.005 & 7.670 \\
SN2016ews & 0.000 & -0.759 & -0.732 & 6.990 \\
SN2016hgw & 0.000 & -0.520 & 0.001 & 8.730 \\
SN2016hnk & 0.018 & -0.778 & -0.589 & -- \\
SN2016hrv & 0.011 & 0.024 & 0.014 & 8.620 \\
SN2016itd & 0.013 & 0.005 & 0.000 & 9.740 \\
SN2017cio & 0.003 & 0.011 & 0.007 & 7.240 \\
SN2017fqo & 0.004 & 0.009 & 0.006 & 8.030 \\
SN2017glq & 0.001 & 0.004 & 0.003 & 7.720 \\
SN2017iro & 0.026 & -0.011 & -0.011 & 8.260 \\
SN2017jfs & 0.046 & 0.140 & 0.113 & 8.680 \\
SN2017ya & 0.000 & 0.002 & -1.881 & 9.130 \\
SN2018acj & 0.000 & -0.017 & -0.017 & -- \\
SN2018cvw & 0.000 & 0.002 & -0.284 & 8.600 \\
SN2018fob & 0.005 & 0.007 & 0.006 & 8.610 \\
SN2018gvt & 0.006 & 0.009 & 0.001 & 7.710 \\
SN2018hrq & 0.060 & 0.016 & 0.005 & 9.670 \\
SN2018kbh & 0.000 & 0.001 & 0.001 & 7.570 \\
SN2018kpo & 0.003 & -0.116 & -0.111 & -- \\
SN2018kva & 0.005 & 0.006 & -0.591 & 7.800 \\
SNf20080514-002 & 0.000 & 0.002 & -0.155 & 8.330 \\
SNf20080612-003 & 0.006 & 0.002 & 0.004 & 8.890 \\
iPTF13dkl & 0.001 & 0.001 & 0.009 & 6.870 \\
iPTF13dkx & 0.002 & 0.005 & 0.008 & 6.920 \\
iPTF13ez & 0.019 & 0.031 & 0.012 & 8.920 \\
iPTF14bdn & 0.001 & 0.009 & 0.003 & 7.760 \\
iPTF14gnl & 0.002 & 0.007 & 0.001 & 7.170 \\
iPTF15wb & 0.002 & 0.006 & 0.003 & 9.810
\enddata
\end{deluxetable}


==> pisco_mass_info_full.tex <==
\begin{deluxetable}{lrrrr}
\tablecaption{Global mass in $\log_{10}(M/M_{\odot})$. FAST++, ZPEG masses limited to SDSS or SDSS+GALEX coverage. } \rotate \label{table:sfr}
\tablehead{\colhead{Galaxy} & \colhead{STARLIGHT Mass} & \colhead{Fast++ Mass} & \colhead{ZPEG Mass} & \colhead{Fast++ GALEX Mass}}
\startdata
2MASSJ00164451 & 10.094 & 10.200 & 10.765 & -- \\
2MASSJ00235669 & 9.653 & 9.790 & 10.192 & 9.770 \\
2MASSJ23243021 & 10.219 & 9.910 & 10.452 & 9.890 \\
2MASXJ22532475 & 9.891 & 9.960 & 10.348 & 10.300 \\
2MASXJ00234829 & 10.539 & 9.850 & 10.829 & 9.860 \\
2MASXJ01144386 & 10.434 & 10.300 & 10.723 & 10.430 \\
2MASXJ01403375 & 10.640 & 10.760 & 11.262 & 11.000 \\
2MASXJ02305208 & 10.013 & 9.660 & 10.787 & 10.300 \\
2MASXJ04424248 & 11.023 & -- & -- & -- \\
2MASXJ07192718 & 9.939 & -- & -- & -- \\
2MASXJ08374557 & 9.387 & 9.710 & 9.436 & 9.980 \\
2MASXJ09591230 & 9.826 & -- & -- & -- \\
2MASXJ10525434 & 10.147 & 9.780 & 10.787 & -- \\
2MASXJ12095669 & 10.285 & 10.410 & 10.816 & -- \\
2MASXJ12385810 & 10.638 & 9.900 & 10.844 & 9.840 \\
2MASXJ15024995 & 9.311 & 9.490 & 9.938 & -- \\
2MASXJ15393305 & 10.996 & 11.150 & 11.530 & 11.090 \\
2MASXJ15570268 & 9.839 & 10.080 & 10.082 & 10.080 \\
2MASXJ16065563 & 10.163 & 10.050 & 10.500 & 10.240 \\
2MASXJ16152860 & 9.807 & 9.950 & 10.207 & 10.030 \\
2MASXJ16301506 & 10.725 & 10.450 & 10.910 & 10.390 \\
2MASXJ17100856 & 10.202 & 10.170 & 10.605 & 10.160 \\
2MASXJ18242915 & 9.475 & -- & -- & -- \\
2MASXJ21352164 & 11.302 & 11.160 & 11.360 & 11.200 \\
2MASXJ23024668 & 10.675 & 10.640 & 11.161 & 10.650 \\
2MFGC13321 & 10.496 & -- & -- & -- \\
ANON. & 10.750 & -- & -- & -- \\
ARP143 & 10.057 & 10.870 & 11.080 & 10.880 \\
ARP70 & 11.141 & 11.050 & 11.327 & 10.990 \\
CGCG004-035 & 10.573 & 10.680 & 11.138 & 11.060 \\
CGCG008-023 & 10.355 & 10.330 & 10.604 & 10.270 \\
CGCG042-196 & 10.215 & 10.130 & 10.454 & -- \\
CGCG047-117 & 10.359 & 10.900 & 11.312 & 10.580 \\
CGCG064-017 & 9.707 & 9.820 & 10.365 & -- \\
CGCG092-024 & 10.359 & 10.140 & 10.137 & 10.210 \\
CGCG107-031 & 10.551 & 10.610 & 11.068 & 10.540 \\
CGCG207-042 & 10.006 & 10.200 & 10.817 & 10.470 \\
CGCG229-009 & 10.478 & -- & -- & -- \\
CGCG229-010 & 10.045 & -- & -- & -- \\
CGCG308-009 & 10.489 & 10.600 & 11.070 & 10.450 \\
CGCG476117 & 9.973 & 10.200 & 10.724 & 9.870 \\
FGC175A & 10.048 & 10.340 & 10.720 & 10.270 \\
GALEXASCJ012052 & 8.530 & 8.580 & 8.995 & 8.950 \\
GALEXASCJ161311 & 9.929 & -- & -- & -- \\
GALEXASCJ234457 & 10.298 & 9.310 & 9.626 & 9.310 \\
IC0208 & 9.980 & 9.730 & 10.382 & 9.970 \\
IC0391 & 9.504 & -- & -- & -- \\
IC0701 & 9.874 & 9.890 & 10.279 & 9.720 \\
IC0758 & 8.518 & 8.960 & 9.333 & 8.850 \\
IC1481 & 10.176 & 10.550 & 10.952 & 10.570 \\
IC1890 & 11.413 & 11.390 & 11.916 & 11.630 \\
IC2373 & 9.353 & 9.630 & 10.083 & 9.780 \\
IC2481 & 9.747 & 10.150 & 10.482 & 10.180 \\
IC3918 & 9.062 & 9.160 & 9.571 & 9.120 \\
IC4526 & 10.725 & 10.670 & 10.958 & 10.670 \\
IC4582 & 9.573 & 8.630 & 9.609 & 8.630 \\
IZW45 & 10.245 & 10.260 & 10.729 & -- \\
KUG0147+328B & 9.357 & 9.320 & 9.815 & 9.510 \\
KUG0210-078 & 10.083 & 10.420 & 10.660 & 10.260 \\
LEDA1709570 & 9.417 & 9.010 & 9.962 & 9.020 \\
M82 & -- & -- & -- & -- \\
MCG+02-58-008 & 11.324 & 11.140 & 11.599 & -- \\
MCG+03-30-38 & 9.647 & -- & -- & -- \\
MCG+05-30-111 & 9.119 & -- & -- & -- \\
MCG+07-05-39 & 9.734 & -- & -- & -- \\
MCG+08-01-03 & 9.255 & -- & -- & -- \\
MCG+08-10-07 & 10.196 & -- & -- & -- \\
MCG+08-19-17 & 9.743 & 9.280 & 10.194 & -- \\
MCG+08-36-16 & 10.427 & -- & -- & -- \\
MCG+09-22-53 & 9.372 & 8.960 & 9.318 & -- \\
MCG+11-08-25 & 10.016 & -- & -- & -- \\
MCG+11-10-34 & 10.089 & -- & -- & -- \\
MCG-01-09-006 & 10.838 & 10.160 & 11.188 & 10.150 \\
MCG-01-10-019 & 10.044 & 9.820 & 10.456 & 10.000 \\
MCG-01-33-12 & 9.800 & 10.290 & 10.603 & 10.310 \\
MCG-01-54-016 & 8.926 & 8.560 & 9.321 & 8.510 \\
MCG-02-02-086 & 11.613 & 11.800 & 12.076 & 11.690 \\
NGC0105 & 10.206 & 10.340 & 10.701 & 9.950 \\
NGC0214 & 10.956 & 10.770 & 10.994 & 10.630 \\
NGC0224A & -inf & -- & -- & -- \\
NGC0309 & 10.505 & 10.930 & 11.175 & 10.790 \\
NGC0495 & 10.649 & 10.640 & 11.102 & 10.530 \\
NGC0523 & 10.335 & 10.620 & 10.906 & 10.540 \\
NGC0628 & 9.925 & -- & -- & -- \\
NGC0691 & 10.234 & 10.630 & 11.097 & 10.660 \\
NGC0716 & 10.422 & 10.530 & 10.805 & 10.110 \\
NGC0774 & 10.781 & 10.680 & 11.182 & 10.650 \\
NGC0776 & 10.706 & 10.680 & 10.911 & 10.740 \\
NGC0890 & 11.126 & -- & -- & -- \\
NGC0932 & 11.029 & 10.990 & 11.511 & 11.150 \\
NGC0938 & 10.813 & 10.790 & 11.348 & 10.830 \\
NGC0976 & 10.991 & 10.890 & 11.091 & 10.860 \\
NGC0991 & 9.222 & 9.310 & 9.767 & 9.310 \\
NGC1056 & 9.944 & 9.970 & 10.450 & -- \\
NGC1058 & 8.820 & -- & -- & -- \\
NGC1060 & 11.624 & 11.450 & 11.924 & 11.490 \\
NGC1070 & 10.969 & 11.010 & 11.303 & 11.010 \\
NGC1093 & 10.379 & 10.290 & 10.437 & 10.390 \\
NGC1142 & 11.420 & 11.530 & 11.741 & 11.450 \\
NGC1259 & 10.813 & 10.550 & 10.874 & 10.320 \\
NGC1590 & 9.994 & 9.690 & 10.585 & 9.710 \\
NGC1637 & 9.370 & -- & -- & -- \\
NGC1667 & 10.834 & 10.870 & 11.090 & 10.750 \\
NGC2276A & -- & -- & -- & -- \\
NGC2276E & -- & -- & -- & -- \\
NGC2276F & -- & -- & -- & -- \\
NGC2315 & 11.156 & -- & -- & -- \\
NGC2320 & 11.412 & -- & -- & -- \\
NGC2333 & 10.553 & -- & -- & -- \\
NGC2347 & 10.799 & -- & -- & -- \\
NGC2431 & 10.529 & -- & -- & -- \\
NGC2526 & 9.849 & 10.240 & 10.472 & -- \\
NGC2554 & 10.994 & 10.980 & 11.575 & 10.990 \\
NGC2565 & 10.608 & 10.140 & 10.408 & 10.180 \\
NGC2577 & 10.057 & 9.960 & 10.550 & 9.990 \\
NGC2595 & 10.650 & 10.790 & 11.172 & 10.460 \\
NGC2596 & 10.324 & 10.620 & 11.003 & 10.630 \\
NGC2604 & 9.197 & 9.110 & 9.656 & 9.820 \\
NGC2618 & 10.484 & 10.860 & 11.075 & 10.850 \\
NGC2623 & 10.329 & 10.360 & 10.891 & 10.180 \\
NGC2639 & 10.893 & 10.730 & 11.281 & 10.660 \\
NGC2691 & 10.075 & 10.390 & 10.688 & 10.200 \\
NGC2748 & 9.395 & -- & -- & -- \\
NGC2765 & 10.444 & 10.760 & 11.403 & 10.850 \\
NGC2771 & 10.530 & 10.620 & 10.852 & 10.610 \\
NGC2789 & 10.582 & 10.730 & 11.066 & 10.720 \\
NGC2906 & 10.243 & 9.920 & 10.149 & 9.850 \\
NGC2916 & 10.490 & 10.440 & 10.730 & 10.270 \\
NGC2926 & 9.845 & 9.950 & 10.261 & 9.890 \\
NGC3057 & 8.834 & 8.860 & 9.475 & 8.680 \\
NGC3158 & 11.464 & 11.440 & 12.047 & 11.420 \\
NGC3184 & 9.408 & -- & -- & -- \\
NGC3310 & 9.775 & 9.360 & 10.120 & 9.250 \\
NGC3323 & 9.648 & 9.670 & 10.087 & 9.490 \\
NGC3451 & 9.100 & 9.310 & 9.642 & 8.920 \\
NGC3499 & 9.575 & 9.260 & 9.674 & -- \\
NGC3655 & 9.899 & 9.980 & 10.204 & 9.890 \\
NGC3687 & 9.992 & 10.110 & 10.522 & 10.030 \\
NGC3811 & 10.205 & 10.260 & 10.671 & 9.920 \\
NGC3847 & 11.150 & 11.140 & 11.729 & 11.080 \\
NGC3861 & 10.466 & 10.600 & 10.974 & 10.290 \\
NGC3905 & 10.755 & -- & -- & -- \\
NGC3913 & 8.611 & 9.340 & 9.667 & -- \\
NGC3982 & 8.526 & 9.890 & 10.205 & -- \\
NGC4070 & 10.973 & 11.190 & 11.693 & 11.180 \\
NGC4210 & 10.181 & 9.530 & 10.478 & 9.690 \\
NGC4384 & 9.393 & 9.820 & 10.143 & 9.450 \\
NGC4470 & 9.597 & 10.130 & 10.398 & 9.970 \\
NGC4644 & 10.269 & 10.210 & 10.472 & -- \\
NGC4866 & 10.560 & 10.380 & 10.949 & 10.330 \\
NGC4874 & 11.454 & 11.510 & 12.100 & 11.420 \\
NGC4961 & 9.416 & 9.670 & 9.961 & 9.310 \\
NGC5000 & 10.717 & 10.550 & 10.888 & 10.650 \\
NGC5056 & 10.264 & 10.520 & 10.918 & 10.370 \\
NGC5157 & 10.931 & 10.840 & 10.976 & 11.040 \\
NGC5338 & 8.516 & 9.520 & 9.757 & 9.520 \\
NGC5339 & 10.118 & 10.230 & 10.794 & 10.490 \\
NGC5378 & 10.355 & 10.250 & 10.728 & 10.240 \\
NGC5406 & 10.667 & 10.880 & 11.175 & 10.850 \\
NGC5410 & 9.551 & 9.440 & 9.905 & 9.250 \\
NGC5421 & 10.805 & 10.900 & 11.182 & 10.740 \\
NGC5425 & 9.178 & 8.980 & 9.410 & 8.990 \\
NGC5426 & 10.011 & -- & -- & -- \\
NGC5468 & 9.866 & -- & -- & -- \\
NGC5480 & 9.588 & 9.510 & 10.163 & -- \\
NGC5525 & 10.952 & 10.970 & 11.517 & 10.960 \\
NGC5557 & 11.146 & 10.900 & 11.487 & 10.930 \\
NGC5559 & 10.322 & 10.320 & 10.703 & 10.380 \\
NGC5587 & 10.279 & 10.270 & 10.771 & 10.390 \\
NGC5611 & 9.770 & 9.620 & 10.221 & 9.610 \\
NGC5630 & 9.213 & 9.490 & 9.950 & 9.420 \\
NGC5668 & 10.337 & 9.540 & 9.775 & 9.550 \\
NGC5682 & 8.912 & 9.420 & 9.762 & 9.120 \\
NGC5714 & 9.692 & 9.350 & 9.873 & 9.160 \\
NGC5732 & 9.568 & 9.960 & 10.302 & 9.890 \\
NGC5735 & 10.177 & 9.990 & 10.758 & 10.040 \\
NGC5772 & 10.864 & 10.760 & 10.994 & 10.520 \\
NGC5829 & 10.122 & 10.380 & 10.778 & 10.300 \\
NGC5837 & 10.733 & 10.680 & 11.005 & 10.700 \\
NGC5888 & 11.291 & 11.210 & 11.415 & 10.900 \\
NGC5910 & 11.476 & 11.680 & 12.123 & 11.570 \\
NGC5980 & 10.706 & 10.540 & 10.889 & 10.700 \\
NGC5996 & 9.749 & 9.890 & 10.211 & 9.510 \\
NGC6063 & 9.691 & 9.670 & 10.167 & 9.560 \\
NGC6146 & 11.417 & 11.350 & 11.932 & 11.340 \\
NGC6166 & 11.591 & 11.630 & 12.087 & 11.580 \\
NGC6173 & 11.598 & 11.400 & 12.061 & 11.360 \\
NGC6186 & 10.210 & 10.300 & 10.748 & -- \\
NGC6261 & 10.867 & 11.310 & 11.715 & 11.210 \\
NGC6373 & 9.129 & 8.820 & 9.314 & 8.830 \\
NGC6643 & 10.084 & -- & -- & -- \\
NGC6786 & 10.878 & -- & -- & -- \\
NGC6946 & -- & -- & -- & -- \\
NGC6962 & 11.007 & 11.060 & 11.645 & 11.030 \\
NGC7033 & 10.882 & -- & -- & -- \\
NGC7042 & 10.852 & -- & -- & -- \\
NGC7047 & 10.620 & 10.570 & 11.051 & 10.450 \\
NGC7222 & 10.791 & 11.290 & 11.553 & 11.390 \\
NGC7253 & 10.166 & 10.630 & 10.947 & 10.630 \\
NGC7311 & 11.064 & 10.960 & 11.478 & 10.930 \\
NGC7319 & 11.132 & 10.870 & 11.247 & 11.000 \\
NGC7321 & 10.697 & 10.950 & 11.221 & 10.580 \\
NGC7364 & 10.667 & 10.740 & 11.001 & 10.470 \\
NGC7461 & 10.016 & 10.660 & 11.082 & -- \\
NGC7469 & 10.910 & 10.060 & 11.005 & 10.050 \\
NGC7489 & 10.514 & 10.410 & 10.899 & 10.530 \\
NGC7503 & 11.366 & 11.680 & 12.093 & 11.540 \\
NGC7619 & 11.265 & 11.360 & 11.927 & 11.310 \\
NGC7653 & 10.342 & 10.510 & 11.004 & 10.520 \\
NGC7691 & 10.339 & 10.460 & 10.850 & 10.460 \\
NGC7771 & 10.923 & 11.150 & 11.413 & 10.950 \\
NGC7803 & 10.594 & 10.820 & 11.062 & 10.470 \\
PGC0010652 & 11.129 & -- & -- & -- \\
PGC0014370 & 9.528 & -- & -- & -- \\
PGC0035860 & 8.570 & 8.620 & 8.891 & 8.760 \\
PGC0213858 & 9.539 & 9.520 & 10.053 & 9.520 \\
PGC063016 & 10.072 & -- & -- & -- \\
PGC067911 & 9.504 & -- & -- & -- \\
PGC10738 & 11.067 & -- & -- & -- \\
PGC11179 & 10.906 & 10.840 & 11.345 & 11.050 \\
PGC1481751 & 10.287 & 10.450 & 10.728 & 10.390 \\
PGC213672 & 10.197 & 10.260 & 10.555 & 10.370 \\
PGC3086846 & 9.372 & 9.230 & 9.886 & 9.250 \\
PGC34730 & 9.566 & 9.670 & 10.003 & -- \\
PGC37426 & 9.502 & 9.940 & 10.549 & 9.970 \\
PGC74050 & 9.462 & -- & -- & -- \\
SDSSJ004750 & 10.113 & 9.370 & 10.626 & 9.290 \\
SDSSJ02595365 & 9.877 & -- & -- & -- \\
SDSSJ083516 & 9.190 & 9.380 & 9.737 & 9.670 \\
SDSSJ08535700 & 10.401 & 9.500 & 10.426 & 9.490 \\
SDSSJ120951251947165 & 10.147 & 10.170 & 10.489 & 10.220 \\
SDSSJ161812 & 8.867 & 9.230 & 9.662 & 9.260 \\
SDSSJ170413 & 10.098 & 9.790 & 10.813 & 10.540 \\
UGC00005 & 10.677 & 10.300 & 11.089 & 10.300 \\
UGC00040 & 10.807 & 10.520 & 11.094 & 10.420 \\
UGC00139 & 9.911 & 9.740 & 10.176 & 10.010 \\
UGC00148 & 10.184 & 10.150 & 10.460 & -- \\
UGC01087 & 10.125 & 9.730 & 10.630 & -- \\
UGC02134 & 10.475 & 9.790 & 10.742 & 10.660 \\
UGC02175 & 9.567 & -- & -- & -- \\
UGC02308 & 10.570 & 10.670 & 11.003 & 10.670 \\
UGC02628 & 10.527 & 9.990 & 10.902 & 10.190 \\
UGC02756 & 9.813 & 10.780 & 11.219 & -- \\
UGC02829 & 10.792 & 10.780 & 11.363 & 10.860 \\
UGC02836 & 10.387 & 10.610 & 10.911 & 10.720 \\
UGC02912 & 10.772 & -- & -- & -- \\
UGC02931 & 9.839 & -- & -- & -- \\
UGC03108 & 10.282 & -- & -- & -- \\
UGC03151 & 10.732 & 10.110 & 11.199 & -- \\
UGC03312 & 10.155 & -- & -- & -- \\
UGC03513 & 9.876 & -- & -- & -- \\
UGC03552 & 9.585 & 9.980 & 10.244 & 10.340 \\
UGC03555 & 10.584 & -- & -- & -- \\
UGC03611 & 10.109 & -- & -- & -- \\
UGC03627 & 9.882 & -- & -- & -- \\
UGC03770 & 10.706 & -- & -- & -- \\
UGC03843 & 9.128 & -- & -- & -- \\
UGC03944 & 9.690 & 9.960 & 10.354 & 10.000 \\
UGC04008 & 11.161 & 11.110 & 11.278 & 10.970 \\
UGC04036 & 10.169 & -- & -- & -- \\
UGC04107 & 10.029 & 10.000 & 10.609 & -- \\
UGC04132 & 10.893 & 10.390 & 10.947 & 10.580 \\
UGC04179 & 9.400 & 9.670 & 9.976 & 9.480 \\
UGC04195 & 10.407 & 10.500 & 10.611 & 10.480 \\
UGC04308 & 9.934 & 9.420 & 10.425 & 10.440 \\
UGC04310 & 9.453 & 9.480 & 9.977 & 9.410 \\
UGC04414 & 10.799 & 10.880 & 11.410 & 10.800 \\
UGC04423 & 9.082 & -- & -- & -- \\
UGC04455 & 10.728 & 10.730 & 10.966 & 10.860 \\
UGC04461 & 9.849 & 9.940 & 10.269 & 9.610 \\
UGC04468 & 10.613 & 10.880 & 11.531 & 10.880 \\
UGC04981 & 9.381 & -- & -- & -- \\
UGC05100 & 11.396 & 10.270 & 10.784 & 10.040 \\
UGC05129 & 10.132 & 10.240 & 10.501 & 10.210 \\
UGC05392 & 9.847 & 9.920 & 10.175 & -- \\
UGC05520 & 9.497 & 9.620 & 9.936 & -- \\
UGC05695 & 9.227 & 9.290 & 9.946 & 9.440 \\
UGC06036 & 11.081 & 10.870 & 11.302 & 10.790 \\
UGC06517 & 9.341 & 9.620 & 9.928 & 9.380 \\
UGC07228 & 10.271 & 10.490 & 10.833 & 10.180 \\
UGC08250 & 9.843 & 9.740 & 10.315 & 9.890 \\
UGC08472 & 10.607 & 10.340 & 10.980 & 10.580 \\
UGC08503 & 9.190 & 9.310 & 9.750 & 9.160 \\
UGC08733 & 9.015 & 9.520 & 9.835 & 9.420 \\
UGC08932 & 8.996 & 9.020 & 9.331 & 8.740 \\
UGC09165 & 10.304 & 9.880 & 10.761 & 9.830 \\
UGC09356 & 9.331 & 8.970 & 9.277 & 8.930 \\
UGC09842 & 10.465 & 10.580 & 10.843 & 10.590 \\
UGC10064 & 10.257 & 10.640 & 11.101 & 10.510 \\
UGC10097 & 11.252 & 11.110 & 11.649 & -- \\
UGC10123 & 10.116 & 10.330 & 10.737 & 10.080 \\
UGC10331 & 9.833 & 9.840 & 10.164 & 9.720 \\
UGC10414 & 10.040 & 10.150 & 11.291 & 10.160 \\
UGC1071 & 10.691 & 10.460 & 10.762 & 10.460 \\
UGC11064 & 10.035 & -- & -- & -- \\
UGC11162 & 9.257 & -- & -- & -- \\
UGC11260 & 10.522 & -- & -- & -- \\
UGC11723 & 10.128 & 10.230 & 10.563 & 10.250 \\
UGC11758 & 11.025 & -- & -- & -- \\
UGC11922 & 10.038 & -- & -- & -- \\
UGC11975 & 10.382 & -- & -- & -- \\
UGC12157 & 10.056 & 9.250 & 10.341 & -- \\
UGC12809 & 10.679 & -- & -- & -- \\
UGC12810 & 10.653 & 10.500 & 10.875 & 10.510 \\
UGC12850 & 9.878 & 10.180 & 10.500 & -- \\
UGC2164 & 10.416 & 10.650 & 11.113 & 10.680 \\
UGC3236 & 10.550 & -- & -- & -- \\
UGC6837 & 9.263 & 9.390 & 10.005 & 9.320
\enddata
\end{deluxetable}


==> pisco_sfr_info_full.tex <==
\begin{deluxetable}{lrrrrr}
\tablecaption{Global SFR in $M_{\odot}\text{yr}^{-1}$.\rotate \label{table:sfr}}
\tablehead{\colhead{Galaxy} & \colhead{FAST++ SFR} & \colhead{H$\alpha$ SFR} & \colhead{NUV SFR} & \colhead{FUV SFR} & \colhead{ZPEG SFR}}
\startdata
2MASXJ22532475 & 0.692 & 0.395 & 1.253 & 0.577 & 0.000 \\
2MASXJ00234829 & 141.254 & 3.910 & 20.854 & 10.341 & 124.738 \\
2MASXJ01144386 & 3.388 & 1.692 & 2.822 & 1.638 & 13.274 \\
2MASXJ08374557 & 10.715 & 1.649 & 3.722 & 1.596 & 16.866 \\
2MASXJ15570268 & 0.741 & 0.010 & 0.367 & 0.211 & 10.864 \\
2MASXJ16152860 & 0.724 & 0.108 & 0.981 & 0.538 & 0.551 \\
2MASXJ16301506 & 27.542 & 1.632 & 3.108 & 2.095 & 19.861 \\
2MASXJ17100856 & 0.020 & 0.034 & 0.268 & 0.245 & 1.782 \\
2MASXJ23024668 & 0.000 & 0.263 & 0.105 & 0.075 & 4.634 \\
ARP143 & 4.898 & 1.482 & 5.137 & 3.094 & 5.383 \\
ARP70 & 26.303 & 1.215 & 4.171 & 2.908 & 7.194 \\
CGCG004-035 & 3.890 & 0.542 & 2.596 & 1.455 & 5.012 \\
CGCG008-023 & 1.318 & 2.253 & 6.753 & 3.583 & 1.315 \\
CGCG047-117 & 64.565 & 3.356 & 5.592 & 3.931 & 14.454 \\
CGCG107-031 & 0.380 & 0.029 & 0.415 & 0.352 & 0.000 \\
CGCG207-042 & 3.467 & 1.071 & 3.151 & 2.100 & 40.832 \\
CGCG308-009 & 0.209 & 0.023 & 0.185 & 0.144 & 0.000 \\
CGCG476117 & 51.286 & 1.193 & 2.242 & 1.362 & 8.433 \\
FGC175A & 0.155 & 0.260 & 1.076 & 1.318 & 1.239 \\
GALEXASCJ012052 & 1.202 & 0.176 & 1.806 & 1.020 & 1.622 \\
GALEXASCJ234457 & 30.903 & 0.495 & 3.326 & 2.141 & 26.363 \\
IC0208 & 2.291 & 0.245 & 1.071 & 0.623 & 6.180 \\
IC0701 & 11.749 & 2.350 & 2.752 & 1.749 & 8.610 \\
IC0758 & 4.677 & 0.044 & 0.160 & 0.116 & 6.353 \\
IC1481 & 3.020 & 1.411 & 6.567 & 2.494 & 19.588 \\
IC2373 & 1.738 & 1.171 & 6.817 & 3.865 & 1.125 \\
IC2481 & 0.000 & 1.210 & 0.059 & 0.000 & 5.598 \\
IC3918 & 2.630 & 1.015 & 4.526 & 2.893 & 1.122 \\
IC4526 & 2.630 & 2.861 & 10.273 & 5.628 & 25.882 \\
IC4582 & 5.370 & 0.181 & 0.733 & 0.420 & 0.585 \\
KUG0147+328B & 0.398 & 0.240 & 1.002 & 0.639 & 0.873 \\
KUG0210-078 & 1.950 & 0.451 & 1.293 & 0.884 & 1.811 \\
MCG+08-19-17 & -- & 2.115 & 0.000 & 0.000 & 3.006 \\
MCG-01-09-006 & 281.838 & 2.320 & 4.556 & 3.642 & 151.705 \\
MCG-01-10-019 & 0.174 & 0.821 & 0.724 & 0.706 & 2.723 \\
MCG-01-33-12 & 2.089 & 0.166 & 0.615 & 0.415 & 0.740 \\
MCG-01-54-016 & 5.495 & 0.209 & 5.707 & 2.652 & 1.371 \\
MCG-02-02-086 & 38.905 & 0.365 & 13.256 & 5.626 & 331.131 \\
NGC0105 & 61.660 & 2.157 & 4.688 & 2.817 & 4.624 \\
NGC0214 & 22.387 & 2.784 & 5.437 & 2.969 & 25.351 \\
NGC0309 & 8.318 & 3.288 & 8.799 & 5.812 & 22.542 \\
NGC0495 & 2.188 & 0.007 & 0.531 & 0.322 & 3.436 \\
NGC0523 & 2.692 & 1.394 & 3.202 & 1.698 & 3.258 \\
NGC0691 & 1.549 & 0.206 & 6.438 & 1.171 & 0.000 \\
NGC0716 & 70.795 & 3.020 & 5.087 & 2.436 & 1.416 \\
NGC0774 & 0.000 & 0.058 & 0.192 & 0.204 & 0.000 \\
NGC0776 & 2.884 & 2.288 & 6.513 & 3.995 & 1.824 \\
NGC0932 & 5.495 & 0.446 & 2.117 & 1.160 & 0.000 \\
NGC0938 & 5.248 & 0.211 & 1.042 & 0.540 & 0.000 \\
NGC0976 & 7.413 & 3.414 & 5.542 & 3.353 & 2.624 \\
NGC0991 & 0.023 & 0.123 & 0.570 & 0.469 & 2.366 \\
NGC1060 & 0.000 & 0.078 & 0.923 & 1.670 & 0.000 \\
NGC1070 & 9.550 & 1.596 & 2.762 & 1.782 & 4.592 \\
NGC1093 & 4.266 & 0.986 & 2.251 & 1.895 & 91.833 \\
NGC1142 & 20.893 & 5.782 & 6.497 & 3.215 & 19.815 \\
NGC1259 & 0.000 & 0.019 & 0.080 & 0.037 & 13.122 \\
NGC1667 & 21.380 & 7.633 & 8.955 & 6.259 & 4.188 \\
NGC2526 & -- & 0.864 & 0.000 & 0.000 & 0.598 \\
NGC2554 & 1.148 & 0.630 & 1.601 & 0.553 & 4.498 \\
NGC2565 & 0.009 & 0.343 & 0.830 & 0.619 & 43.853 \\
NGC2595 & 2.188 & 1.162 & 2.673 & 2.114 & 2.388 \\
NGC2596 & 5.012 & 2.173 & 4.695 & 2.268 & 2.793 \\
NGC2604 & 0.000 & 0.620 & 0.012 & 0.010 & 1.374 \\
NGC2618 & 4.169 & 0.105 & 1.137 & 0.840 & 0.334 \\
NGC2623 & 0.347 & 0.895 & 3.325 & 2.166 & 2.523 \\
NGC2639 & 0.028 & 0.264 & 0.520 & 0.247 & 0.000 \\
NGC2691 & 1.660 & 0.949 & 2.025 & 0.718 & 1.038 \\
NGC2765 & 0.000 & 0.019 & 0.178 & 0.153 & 7.586 \\
NGC2771 & 2.884 & 0.792 & 1.388 & 0.871 & 0.203 \\
NGC2789 & 0.589 & 1.258 & 1.800 & 0.593 & 3.491 \\
NGC2906 & 0.437 & 0.511 & 0.659 & 0.414 & 0.039 \\
NGC2916 & 2.042 & 1.417 & 2.076 & 1.498 & 1.600 \\
NGC2926 & 3.981 & 0.880 & 1.096 & 0.754 & 2.582 \\
NGC3057 & 2.884 & 0.145 & 0.646 & 0.475 & 0.750 \\
NGC3158 & 4.677 & 0.131 & 2.085 & 0.798 & 0.000 \\
NGC3310 & 29.512 & 1.965 & 4.861 & 3.256 & 3.357 \\
NGC3323 & 12.303 & 2.488 & 4.453 & 2.559 & 6.855 \\
NGC3451 & 2.089 & 0.270 & 0.334 & 0.205 & 0.944 \\
NGC3655 & 0.490 & 0.773 & 1.608 & 0.641 & 0.540 \\
NGC3687 & 10.233 & 0.338 & 0.788 & 0.528 & 6.761 \\
NGC3811 & 0.174 & 1.400 & 2.000 & 1.405 & 2.118 \\
NGC3861 & 2.239 & 0.822 & 1.615 & 1.133 & 1.510 \\
NGC4070 & 1.122 & 0.336 & 1.591 & 0.589 & 51.761 \\
NGC4384 & 6.310 & 0.885 & 0.687 & 0.428 & 1.219 \\
NGC4470 & 2.089 & 0.704 & 2.095 & 1.248 & 3.767 \\
NGC4866 & 0.295 & 0.043 & 0.342 & 0.143 & 0.000 \\
NGC4874 & 0.001 & 0.039 & 2.126 & 0.796 & 0.000 \\
NGC4961 & 0.724 & 0.431 & 1.848 & 1.275 & 0.733 \\
NGC5000 & 3.388 & 1.610 & 2.503 & 1.490 & 4.276 \\
NGC5056 & 4.786 & 2.688 & 6.902 & 4.813 & 13.836 \\
NGC5157 & 17.783 & 0.555 & 2.524 & 1.356 & 155.955 \\
NGC5339 & 2.570 & 0.444 & 1.843 & 1.043 & 7.925 \\
NGC5378 & 0.182 & 0.170 & 0.350 & 0.285 & 1.146 \\
NGC5406 & 10.715 & 1.555 & 2.771 & 1.784 & 5.689 \\
NGC5421 & 0.912 & 1.046 & 1.920 & 1.135 & 8.995 \\
NGC5525 & 1.000 & 0.064 & 0.927 & 0.316 & 8.810 \\
NGC5557 & 0.000 & 0.017 & 0.331 & 0.171 & 0.000 \\
NGC5559 & 1.445 & 1.205 & 7.061 & 2.519 & 0.828 \\
NGC5587 & 1.230 & 0.114 & 0.486 & 0.245 & 0.991 \\
NGC5630 & 3.388 & 0.806 & 4.300 & 2.396 & 1.910 \\
NGC5668 & 1.950 & 4.334 & 7.090 & 4.452 & 2.761 \\
NGC5682 & 0.537 & 0.201 & 0.469 & 0.306 & 0.575 \\
NGC5714 & 2.512 & 0.190 & 1.582 & 0.857 & 0.173 \\
NGC5732 & 2.399 & 0.553 & 1.063 & 0.630 & 0.288 \\
NGC5735 & 2.630 & 0.759 & 3.574 & 2.248 & 7.834 \\
NGC5772 & 11.482 & 0.652 & 1.845 & 1.142 & 2.080 \\
NGC5829 & 3.311 & 1.147 & 8.632 & 5.431 & 9.795 \\
NGC5837 & 6.761 & 6.452 & 7.960 & 4.227 & 3.690 \\
NGC5888 & 10.000 & 0.940 & 3.364 & 1.996 & 9.795 \\
NGC5980 & 3.311 & 2.366 & 9.712 & 4.476 & 8.913 \\
NGC5996 & 10.965 & 2.143 & 5.368 & 3.219 & 1.419 \\
NGC6063 & 2.692 & 0.342 & 0.747 & 0.626 & 3.548 \\
NGC6166 & 0.000 & 0.150 & 1.813 & 1.307 & 0.000 \\
NGC6186 & -- & 1.012 & 0.000 & 0.000 & 1.845 \\
NGC6261 & 10.000 & 0.121 & 2.655 & 1.526 & 11.614 \\
NGC6373 & 15.136 & 0.298 & 0.631 & 0.589 & 47.206 \\
NGC6962 & 1.202 & 0.131 & 1.532 & 1.246 & 0.000 \\
NGC7047 & 0.550 & 1.621 & 1.717 & 1.622 & 12.972 \\
NGC7222 & 12.882 & 0.899 & 9.286 & 6.163 & 10.375 \\
NGC7253 & 4.677 & 0.772 & 3.842 & 2.976 & 1.510 \\
NGC7311 & 6.918 & 1.155 & 3.561 & 1.836 & 6.982 \\
NGC7319 & 0.631 & 1.784 & 1.254 & 0.780 & 3.855 \\
NGC7321 & 14.454 & 3.225 & 8.679 & 5.582 & 3.581 \\
NGC7364 & 0.437 & 2.378 & 1.780 & 1.128 & 2.104 \\
NGC7469 & 213.796 & 15.445 & 17.964 & 10.955 & 19.011 \\
NGC7489 & 11.482 & 5.320 & 11.012 & 6.542 & 14.655 \\
NGC7619 & 0.000 & 0.035 & 0.728 & 0.428 & 0.000 \\
NGC7691 & 1.445 & 0.774 & 2.046 & 1.540 & 1.426 \\
NGC7771 & 1.148 & 4.994 & 4.970 & 2.522 & 8.318 \\
NGC7803 & 0.692 & 2.230 & 1.189 & 0.651 & 3.776 \\
PGC0035860 & 0.407 & 0.160 & 1.210 & 0.851 & 0.908 \\
PGC11179 & 4.169 & 0.055 & 1.021 & 0.620 & 0.000 \\
PGC1481751 & 0.251 & 0.037 & 0.364 & 0.200 & 2.037 \\
PGC37426 & 0.562 & 0.004 & 0.210 & 0.060 & 0.910 \\
SDSSJ083516 & 0.457 & 0.371 & 8.254 & 3.910 & 0.254 \\
SDSSJ120951251947165 & 2.188 & 1.291 & 2.585 & 1.080 & 5.861 \\
SDSSJ161812 & 0.295 & 0.144 & 0.827 & 0.540 & 0.291 \\
UGC00005 & 144.544 & 4.873 & 9.946 & 4.587 & 2.636 \\
UGC00040 & 0.437 & 0.661 & 1.635 & 2.315 & 26.730 \\
UGC00139 & 0.000 & 0.778 & 0.079 & 0.059 & 3.273 \\
UGC02628 & 0.295 & 1.106 & 4.703 & 4.006 & 12.388 \\
UGC02829 & 14.791 & 0.050 & 2.278 & 2.614 & 4.634 \\
UGC02836 & 2.630 & 4.420 & 6.881 & 4.733 & 3.428 \\
UGC03552 & 1.096 & 0.498 & 1.000 & 0.808 & 18.750 \\
UGC03944 & 1.318 & 0.491 & 1.673 & 1.071 & 0.647 \\
UGC04008 & 7.586 & 3.126 & 5.131 & 2.462 & 8.710 \\
UGC04132 & 5.248 & 3.533 & 11.547 & 5.190 & 22.594 \\
UGC04179 & 0.000 & 0.320 & 0.411 & 0.315 & 0.977 \\
UGC04195 & 1.660 & 0.920 & 2.455 & 1.261 & 0.881 \\
UGC04308 & 0.000 & 0.863 & 0.065 & 0.063 & 50.119 \\
UGC04310 & 0.501 & 0.232 & 1.056 & 0.662 & 0.555 \\
UGC04414 & 0.692 & 0.479 & 0.989 & 0.860 & 0.000 \\
UGC04455 & 2.754 & 0.795 & 3.762 & 1.879 & 3.381 \\
UGC04461 & 0.513 & 1.244 & 9.750 & 6.079 & 1.288 \\
UGC05100 & 4.365 & 1.003 & 10.892 & 6.200 & 8.770 \\
UGC05129 & 1.288 & 0.432 & 0.710 & 0.441 & 0.635 \\
UGC05695 & 2.089 & 0.187 & 0.498 & 0.256 & 5.808 \\
UGC06036 & 0.000 & 0.165 & 0.243 & 0.247 & 3.483 \\
UGC06517 & 1.622 & 0.182 & 0.703 & 0.454 & 0.708 \\
UGC07228 & 0.389 & 2.750 & 2.352 & 1.290 & 1.349 \\
UGC08250 & 3.981 & 0.430 & 3.738 & 1.457 & 3.631 \\
UGC08503 & 0.288 & 0.176 & 0.761 & 0.395 & 0.400 \\
UGC08733 & 1.445 & 0.143 & 0.971 & 0.657 & 1.445 \\
UGC09165 & 131.826 & 1.678 & 13.321 & 3.576 & 12.531 \\
UGC09356 & 0.195 & 0.158 & 0.968 & 0.538 & 0.442 \\
UGC09842 & 6.310 & 4.313 & 6.189 & 3.748 & 2.588 \\
UGC10064 & 0.363 & 0.092 & 0.718 & 0.480 & 3.319 \\
UGC10331 & 0.832 & 1.982 & 6.438 & 3.864 & 1.023 \\
UGC1071 & 2.042 & 0.619 & 0.589 & 0.240 & 2.421 \\
UGC11723 & 0.120 & 0.445 & 0.416 & 0.312 & 0.665 \\
UGC12157 & -- & 1.076 & 0.000 & 0.000 & 102.094 \\
UGC12810 & 4.365 & 3.273 & 3.029 & 2.334 & 1.626 \\
UGC12850 & -- & 0.947 & 0.000 & 0.000 & 3.648 \\
UGC6837 & 52.481 & 0.327 & 0.306 & 0.185 & 47.863
\enddata
\end{deluxetable}


==> pisco_sn_info_full.tex <==
\begin{deluxetable}{llrrrrrrrrrl}
\tablecaption{Properties of SNe Ia considered in this work. Light-curve fit parameters $x_0$, $x_1$ and $c$ were determined using the SALT2 supernova model. } \rotate \label{table:sn_properties}
\tablehead{\colhead{SN} & \colhead{Survey} & \colhead{$\mu$} & \colhead{RA} & \colhead{Dec} & \colhead{z} & \colhead{$x_0$} & \colhead{$x_1$} & \colhead{$c$} & \colhead{M$_\text{B}$} & \colhead{$\mu_{SN} - \mu_{mod}$} & \colhead{Galaxy}}
\startdata
ASASSN-14kd & CSPII & 35.001 & 343.353 & 4.799 & 0.023 & 0.006 & 1.090 & 0.144 & 16.207 & 0.025 & 2MASXJ22532475 \\
ASASSN-14lo & CSPII & 34.700 & 177.969 & 18.546 & 0.020 & 0.007 & -0.487 & 0.093 & 16.032 & 0.012 & UGC6837 \\
ASASSN-14my & CSPII & 34.706 & 174.626 & -8.976 & 0.020 & 0.011 & -0.578 & -0.060 & 15.550 & -0.045 & NGC3774 \\
ASASSN-15cb & CSPII & 36.204 & 189.959 & 3.797 & 0.040 & 0.003 & 0.918 & 0.025 & 17.049 & -0.031 & CGCG042-196 \\
ASASSN-15cd & CSPII & 36.117 & 149.812 & 12.988 & 0.034 & 0.004 & 0.322 & -0.097 & 16.670 & 0.226 & CGCG064-017 \\
ASASSN-15db & CSPII & 33.475 & 236.745 & 17.884 & 0.011 & 0.024 & -0.530 & 0.051 & 14.677 & 0.093 & NGC5996 \\
ASASSN-15dd & CSPII & 34.969 & 235.995 & 19.212 & 0.024 & 0.007 & -1.314 & -0.020 & 16.083 & -0.163 & CGCG107-031 \\
ASASSN-15ga & PS1 & 32.511 & 194.864 & 14.171 & 0.007 & 0.022 & -1.015 & 0.305 & 14.642 & 0.234 & NGC4866 \\
ASASSN-15tz & PS1 & 34.991 & 40.287 & 43.680 & 0.024 & 0.004 & -1.620 & 0.057 & 16.418 & -0.110 & UGC2164 \\
CSP13n & CSPII & 36.367 & 144.967 & 16.918 & 0.048 & 0.003 & 0.607 & -0.051 & 17.019 & -0.264 & CGCG092-024 \\
iPTF13dkl & PS1 & 36.759 & 356.242 & 3.395 & 0.040 & 0.001 & 0.631 & 0.001 & 17.580 & 0.525 & GALEXASCJ234457 \\
iPTF13dym & CSPII & 35.846 & 351.126 & 14.651 & 0.042 & 0.002 & -3.170 & 0.075 & 17.621 & -0.504 & 2MASSJ23243021 \\
iPTF14aaf & CSPII & 37.015 & 219.211 & 6.139 & 0.059 & 0.001 & 0.524 & 0.058 & 18.043 & -0.086 & CGCG047-117 \\
iPTF14bdn & MISC & 34.334 & 202.687 & 32.761 & 0.016 & 0.021 & 1.534 & -0.083 & 14.705 & 0.085 & UGC08503 \\
iPTF14gnl & CSPII & 36.896 & 5.951 & -3.856 & 0.054 & 0.002 & 0.587 & -0.081 & 17.453 & 0.002 & 2MASXJ00234829 \\
LSQ12gef & CSPII & 37.232 & 25.141 & 18.511 & 0.064 & 0.000 & 1.058 & 0.293 & 18.937 & -0.065 & 2MASXJ01403375 \\
LSQ12hzj & CSPII & 35.821 & 149.801 & -9.003 & 0.035 & 0.004 & -0.310 & -0.091 & 16.512 & -0.089 & 2MASXJ09591230 \\
LSQ13vy & CSPII & 36.243 & 241.732 & 3.001 & 0.042 & 0.002 & -1.105 & 0.087 & 17.671 & -0.088 & 2MASXJ16065563 \\
LSQ14ajn & CSPII & 34.918 & 178.877 & 11.924 & 0.021 & 0.006 & -1.950 & 0.017 & 16.273 & 0.113 & PGC37426 \\
LSQ14azy & CSPII & 36.601 & 168.145 & 12.072 & 0.046 & 0.001 & 0.182 & 0.073 & 17.742 & 0.065 & 2MASXJ11123493 \\
LSQ14q & CSPII & 37.456 & 133.488 & 17.328 & 0.067 & 0.001 & -0.430 & -0.094 & 18.160 & 0.062 & SDSSJ08535700 \\
LSQ15aae & CSPII & 36.755 & 247.563 & 5.931 & 0.052 & 0.001 & 1.120 & 0.127 & 17.899 & -0.049 & 2MASXJ16301506 \\
LSQ15agh & CSPII & 37.180 & 163.226 & 23.598 & 0.060 & 0.001 & 0.958 & -0.053 & 17.760 & 0.036 & 2MASXJ10525434 \\
PS15sv & CSPII & 35.651 & 243.299 & 1.592 & 0.033 & 0.005 & 0.319 & -0.031 & 16.423 & -0.173 & GALEXASCJ161311 \\
SN1989a & MISC & 32.926 & 171.992 & 29.510 & 0.009 & 0.046 & -0.104 & -0.010 & 13.848 & -0.103 & NGC3687 \\
SN1993ae & MISC & 34.360 & 22.454 & -1.977 & 0.019 & 0.013 & -1.621 & -0.111 & 15.231 & -0.184 & UGC1071 \\
SN1995bd & MISC & 33.753 & 71.338 & 11.067 & 0.014 & 0.010 & 0.761 & 0.309 & 15.566 & -0.226 & UGC03151 \\
SN1995e & MISC & 33.176 & 117.986 & 73.010 & 0.012 & 0.003 & -0.494 & 0.757 & 16.706 & -0.336 & UGC04036 \\
SN1997cw & MISC & 34.158 & 6.322 & 12.885 & 0.016 & 0.008 & 1.091 & 0.283 & 15.824 & -0.112 & NGC0105 \\
SN1998aq & MISC & 31.741 & 179.108 & 55.129 & 0.004 & 0.219 & -0.372 & -0.181 & 12.146 & 0.425 & NGC3982 \\
SN1999aa & MISC & 34.351 & 126.925 & 21.487 & 0.015 & 0.022 & 1.260 & -0.118 & 14.658 & 0.251 & NGC2595 \\
SN1999ac & MISC & 33.076 & 241.813 & 7.972 & 0.010 & 0.037 & 0.297 & 0.041 & 14.090 & -0.059 & NGC6063 \\
SN1999dk & MISC & 33.836 & 22.862 & 14.285 & 0.014 & 0.019 & -0.003 & 0.011 & 14.806 & -0.068 & UGC01087 \\
SN1999dq & MISC & 33.676 & 38.499 & 20.975 & 0.014 & 0.028 & 0.932 & -0.021 & 14.367 & -0.163 & NGC0976 \\
SN1999ej & MISC & 34.221 & 20.739 & 33.466 & 0.013 & 0.011 & -1.880 & -0.038 & 15.381 & 0.509 & NGC0495 \\
SN1999gd & MISC & 34.646 & 129.603 & 25.759 & 0.019 & 0.003 & -1.031 & 0.345 & 16.913 & 0.026 & NGC2623 \\
SN2000b & MISC & 34.316 & 106.420 & 50.586 & 0.020 & 0.009 & -1.560 & 0.031 & 15.645 & -0.390 & NGC2320 \\
SN2000ce & MISC & 34.552 & 121.289 & 66.788 & 0.016 & 0.003 & 0.375 & 0.482 & 17.010 & 0.278 & UGC04195 \\
SN2000cn & MISC & 34.976 & 269.418 & 27.833 & 0.023 & 0.004 & -2.598 & 0.040 & 16.529 & -0.049 & UGC11064 \\
SN2000fa & MISC & 34.954 & 108.874 & 23.428 & 0.022 & 0.007 & 0.482 & 0.018 & 15.859 & 0.068 & UGC03770 \\
SN2001br & MISC & 34.959 & 277.606 & 34.104 & 0.020 & 0.005 & -1.323 & 0.020 & 16.208 & 0.240 & UGC11260 \\
SN2001en & MISC & 34.119 & 21.345 & 34.025 & 0.015 & 0.016 & -0.779 & -0.058 & 15.008 & 0.064 & NGC0523 \\
SN2001fe & 4SHOOTER2 & 33.998 & 144.488 & 25.495 & 0.014 & 0.023 & 0.769 & -0.060 & 14.590 & 0.010 & UGC05129 \\
SN2001ic & 4SHOOTER2 & 36.113 & 347.681 & 7.570 & 0.043 & 0.002 & -1.464 & 0.020 & 17.385 & -0.284 & NGC7503 \\
SN2002aw & MISC & 34.955 & 249.371 & 40.881 & 0.026 & 0.005 & -0.549 & 0.053 & 16.169 & -0.337 & 2MFGC13321 \\
SN2002ha & MISC & 33.847 & 311.827 & 0.313 & 0.013 & 0.021 & -1.497 & -0.115 & 14.679 & 0.088 & NGC6962 \\
SN2002jg & MISC & 33.947 & 334.870 & 29.385 & 0.014 & 0.002 & -1.869 & 0.596 & 17.200 & 0.055 & NGC7253 \\
SN2003ic & 4SHOOTER2 & 36.453 & 10.459 & -9.305 & 0.055 & 0.002 & -1.651 & -0.039 & 17.566 & -0.479 & MCG-02-02-086 \\
SN2003it & 4SHOOTER2 & 35.123 & 1.452 & 27.453 & 0.024 & 0.005 & -1.621 & -0.015 & 16.311 & 0.027 & UGC00040 \\
SN2003iv & 4SHOOTER2 & 36.034 & 42.530 & 12.846 & 0.034 & 0.003 & -2.080 & -0.119 & 16.965 & 0.190 & PGC10738 \\
SN2004gu & CSP & 36.490 & 191.603 & 11.949 & 0.047 & 0.002 & 1.427 & 0.066 & 17.373 & -0.102 & FGC175A \\
SN2005eq & CSP & 35.708 & 47.205 & -7.033 & 0.028 & 0.005 & 1.513 & -0.041 & 16.224 & 0.239 & MCG-01-09-006 \\
SN2005kc & CSP & 34.021 & 338.531 & 5.568 & 0.014 & 0.010 & -0.812 & 0.113 & 15.480 & 0.125 & NGC7311 \\
SN2005mc & CSP & 35.027 & 126.776 & 21.646 & 0.026 & 0.003 & -2.010 & 0.177 & 16.922 & -0.252 & UGC04414 \\
SN2005w & CSP & 32.886 & 27.691 & 21.760 & 0.008 & 0.036 & -0.448 & 0.063 & 14.111 & 0.211 & NGC0691 \\
SN2006bb & KEPLER & 35.566 & 128.380 & 41.518 & 0.026 & 0.006 & -2.166 & -0.240 & 16.112 & 0.304 & UGC04468 \\
SN2006eu & MISC & 34.874 & 300.713 & 49.317 & 0.023 & 0.002 & -0.773 & 0.453 & 17.449 & -0.124 & MCG+08-36-16 \\
SN2006ev & CSP & 35.641 & 322.747 & 13.989 & 0.028 & 0.003 & -1.356 & 0.051 & 16.997 & 0.231 & UGC11758 \\
SN2006kf & CSP & 34.849 & 55.460 & 8.157 & 0.021 & 0.007 & -2.072 & -0.095 & 15.855 & 0.064 & UGC02829 \\
SN2006n & KEPLER & 34.408 & 92.130 & 64.724 & 0.014 & 0.016 & -1.818 & -0.215 & 14.972 & 0.454 & CGCG308-009 \\
SN2006td & KEPLER & 34.707 & 29.566 & 36.349 & 0.015 & 0.009 & -1.238 & -0.079 & 15.612 & 0.636 & PGC74050 \\
SN2007a & CSP & 34.534 & 6.319 & 12.887 & 0.016 & 0.009 & 0.553 & 0.075 & 15.611 & 0.263 & NGC0105 \\
SN2007bd & CSP & 35.596 & 127.889 & -1.199 & 0.032 & 0.004 & -1.117 & -0.089 & 16.444 & -0.131 & UGC04455 \\
SN2007hj & MISC & 33.897 & 345.450 & 15.586 & 0.013 & 0.009 & -2.432 & 0.090 & 15.585 & 0.165 & NGC7461 \\
SN2007hu & KEPLER & 36.174 & 254.125 & 27.978 & 0.035 & 0.002 & -1.006 & 0.078 & 17.555 & 0.213 & NGC6261 \\
SN2007jd & CSP & 37.648 & 44.972 & 1.161 & 0.073 & 0.000 & -0.911 & 0.044 & 18.898 & 0.067 & SDSSJ02595365 \\
SN2007r & KEPLER & 36.175 & 116.656 & 44.789 & 0.031 & 0.004 & -1.333 & -0.269 & 16.469 & 0.486 & UGC04008 \\
SN2007ux & CSP & 35.739 & 152.333 & 14.992 & 0.032 & 0.002 & -1.999 & 0.059 & 17.242 & 0.000 & PGC213672 \\
SN2008bi & CSP & 34.243 & 128.972 & 0.706 & 0.014 & 0.005 & -2.618 & 0.187 & 16.283 & 0.269 & NGC2618 \\
SN2008bz & CSP & 37.189 & 189.741 & 11.130 & 0.061 & 0.001 & -0.578 & -0.106 & 17.880 & -0.008 & 2MASXJ12385810 \\
SN2008c & CSP & 34.278 & 104.298 & 20.437 & 0.017 & 0.009 & -0.714 & 0.078 & 15.604 & -0.071 & UGC03611 \\
SN2008dr & MISC & 36.264 & 332.715 & 2.108 & 0.040 & 0.002 & -1.536 & 0.003 & 17.495 & 0.016 & NGC7222 \\
SN2008dt & MISC & 35.753 & 254.127 & 27.976 & 0.035 & 0.001 & 0.459 & 0.442 & 18.062 & -0.209 & NGC6261 \\
SN2008ec & MISC & 34.128 & 345.819 & 8.872 & 0.015 & 0.010 & -0.996 & 0.079 & 15.510 & 0.052 & NGC7469 \\
SN2008hv & CSP & 33.843 & 136.892 & 3.392 & 0.014 & 0.022 & -1.242 & -0.116 & 14.625 & -0.004 & NGC2765 \\
SN2008l & MISC & 34.439 & 49.319 & 41.383 & 0.019 & 0.012 & -1.605 & -0.112 & 15.304 & -0.128 & NGC1259 \\
SN2009ad & CSP & 35.528 & 75.889 & 6.660 & 0.028 & 0.006 & 0.199 & -0.114 & 16.047 & 0.060 & UGC3236 \\
SN2009cz & CSP & 34.838 & 138.750 & 29.735 & 0.022 & 0.009 & 0.673 & -0.009 & 15.617 & -0.068 & NGC2789 \\
SN2009ds & CSP & 34.546 & 177.267 & -9.729 & 0.020 & 0.011 & 1.274 & 0.055 & 15.424 & -0.203 & NGC3905 \\
SN2009fv & KEPLER & 35.289 & 247.434 & 40.812 & 0.029 & 0.004 & -0.179 & 0.083 & 16.531 & -0.257 & NGC6173 \\
SN2009gf & SWIFT & 34.493 & 213.905 & 14.280 & 0.019 & 0.006 & -2.738 & 0.027 & 16.029 & -0.127 & NGC5525 \\
SN2009lf & KEPLER & 36.285 & 30.415 & 15.333 & 0.044 & 0.003 & -1.677 & -0.218 & 16.813 & -0.168 & PGC1481751 \\
SN2009p & CSP & 35.354 & 170.162 & -3.546 & 0.026 & 0.003 & 2.004 & 0.311 & 16.942 & 0.049 & PGC34730 \\
SN2011fs & SWIFT & 34.702 & 334.331 & 35.581 & 0.020 & 0.013 & 0.325 & -0.116 & 15.192 & 0.021 & UGC11975 \\
SN2011im & CSPII & 34.052 & 341.102 & -0.162 & 0.015 & 0.010 & -1.532 & 0.121 & 15.672 & -0.012 & NGC7364 \\
SN2012hl & CSPII & 35.634 & 12.574 & 24.532 & 0.033 & 0.001 & -0.390 & 0.330 & 17.732 & -0.169 & LEDA1709570 \\
SN2012id & CSPII & 33.867 & 70.677 & 18.583 & 0.016 & 0.014 & -1.662 & 0.046 & 15.264 & -0.302 & 2MASXJ04424248 \\
SN2012ij & CSPII & 33.664 & 243.299 & 1.592 & 0.011 & 0.011 & -2.486 & 0.146 & 15.545 & 0.282 & MCG+03-30-38 \\
SN2013aj & CSPII & 32.864 & 208.501 & -7.931 & 0.009 & 0.042 & -1.745 & -0.012 & 14.085 & -0.109 & NGC5339 \\
SN2013fw & CSPII & 34.151 & 318.441 & 13.575 & 0.017 & 0.017 & 0.740 & 0.038 & 15.072 & -0.181 & NGC7042 \\
SN2013gv & CSPII & 35.776 & 47.494 & 19.208 & 0.034 & 0.004 & -1.432 & -0.060 & 16.779 & -0.103 & IC1890 \\
SN2013hh & CSPII & 34.393 & 172.260 & 17.232 & 0.013 & 0.002 & 0.197 & 0.569 & 17.171 & 0.647 & UGC06483 \\
SN2013u & CSPII & 35.884 & 150.299 & 0.329 & 0.034 & 0.003 & 1.200 & 0.123 & 17.000 & -0.019 & CGCG008-023 \\
SN2014dl & CSPII & 35.373 & 247.447 & 8.644 & 0.033 & 0.007 & 1.197 & -0.011 & 16.047 & -0.428 & UGC10414 \\
SN2016cvw & PS1 & 36.142 & 341.553 & 10.559 & 0.039 & 0.002 & -1.642 & -0.060 & 17.185 & -0.029 & MCG+02-58-008 \\
SN2016cyt & PS1 & 35.502 & 317.399 & 15.126 & 0.031 & 0.005 & -1.872 & -0.151 & 16.287 & -0.141 & NGC7033 \\
SN2016ews & PS1 & 36.702 & 225.652 & 23.353 & 0.046 & 0.003 & 0.538 & -0.206 & 16.854 & 0.155 & IC4526 \\
SN2016hgw & PS1 & 34.934 & 44.392 & 5.978 & 0.023 & 0.006 & -2.085 & -0.042 & 16.120 & -0.060 & PGC11179 \\
SN2017ya & PS1 & 37.200 & 4.185 & 15.342 & 0.070 & 0.001 & 1.834 & 0.045 & 17.939 & -0.296 & 2MASSJ00164451 \\
SNf20080514-002 & SWIFT & 35.406 & 202.307 & 11.276 & 0.023 & 0.007 & -1.476 & -0.219 & 15.893 & 0.395 & UGC08472
\enddata
\end{deluxetable}

